How cytoskeletal crosstalk makes cells move: bridging cell-free and cell studies

Cell migration is a fundamental process for life and is highly dependent on the dynamical and mechanical properties of the cytoskeleton. Intensive physical and biochemical crosstalk between actin, microtubules, and intermediate filaments ensures their coordination to facilitate and enable migration. In this review we discuss the different mechanical aspects that govern cell migration and provide, for each mechanical aspect, a novel perspective by juxtaposing two complementary approaches to the biophysical study of cytoskeletal crosstalk: live-cell studies (often referred to as top-down studies) and cell-free studies (often referred to as bottom-up studies). We summarize the main findings from both experimental approaches, and we provide our perspective on bridging the two perspectives to address the open questions of how cytoskeletal crosstalk governs cell migration and makes cells move.

==> extra_template/contractility.tex <==
\begin{document}

\section{Contractility}

\subsection{General Mechanisms}
A cell generates contractile forces via the interaction of the cytoskeletal actin network and non-muscle myosin II motor proteins.
Combined with the polymerisation of actin filaments at their plus (barbed) end, the contraction of the actomyosin network allows a cell to produce a rearward flux so that it may propel itself forwards during migration \cite{Pandya2017} \cite{Muntz2022}.
Within migrating cells, forces at the leading edge have been shown to be strong but transient, while forces at the rear of the cell are comparatively weaker yet sustained.
These findings suggest that migration is driven by contractile forces originating from the rear of the leading edge of a cell \cite{Palecek1998}.
\\

\subsection{in vitro}
Reconstitution studies have replicated the mechanical behaviours and alterations in cell shape driven by the intricate dynamics of actin contraction, thereby creating a pathway towards comprehending cell migration \cite{sonal2019}.
Due to the significant influence of dynamic processes within cells, the integration of motor proteins into  in vitro systems has garnered substantial interest in the last twenty years.
However, our understanding of the precise mechanism by which the localised restructuring of actin architecture fine-tunes stress generation within cells, while also regulating the flow of global contractile networks on a larger scale, remains incomplete.
\\

The dynamics of protrusive F-actin networks that propel the forward motion of migrating cells can be replicated using a limited set of constituents to create a system encompassing actin, myosin and ATP.
The capacity of myosin to induce global network contraction relies on the concentration of proteins that crosslink actin in vitro \cite{Alvarado2017} \cite{Janson1991}.
Giant unilamellar vesicles (GUVs) and droplets containing cytoskeletal components are becoming increasing used to unravel the processes of actin network remodeling and contraction \cite{Liu2019} \cite{Tan2018} \cite{Koenderink}.
Efforts to encapsulate contractile actomyosin networks within cell-sized liposome containers have helped to elucidate the physical basis for cell shape regulation \cite{Carvalho2013}.
\\

Incorporating vimentin networks enhances the speed of actomyosin contractility and results in a visibly more compact contracted structure.
This observation is in line with the expected characteristics of a network exhibiting more solid-like attributes, suggesting that vimentin indeed holds a crucial role in a contractile actomyosin network \cite{shen2021}.
\\

Despite the comprehensive study of actomyosin networks, the interactions between actin and microtubules, which are interpenetrating within the cytoskeleton, remain a subject of ongoing investigation.
It has been shown that microtubules are able to modulate contraction forces in an in vitro environment \cite{valentine2005}.
Microtubules facilitate self-organised contraction powered by myosin through the provision of flexural rigidity and increased connectivity to actin networks \cite{Lee2021}.
The introduction of myosin motors to reconstituted actin networks has been demonstrated to amplify the magnitude and alter the temporal patterns of microtubule bending fluctuations \cite{brangwynne2008}.

\subsection{Cell work}
Historically, the majority of what we know about the contractile forces involved in cell migration is determined from experiments on cells cultured on 2D substrates \cite{Hawkins}.
In these studies, cells are adhered to substrates with known mechanical properties, such as polyacrylamide or PDMS, with embedded fluorescent tracer particles.
By measuring the displacements of these particles with fluroescence microscopy, the traction forces exerted on the susbstrate are computationally extracted using continiuum mechanics models.
The elastic modulus of the substrate may be tuned by altering the concentrations of monomer and crosslinks, enabling use to create biomimetic surfaces which physiologically match the stiffness of biological tissues found in the body.
Recently, viscoelastic polyacrylamide has been used to measure the effect of viscoelastic substrates on cellular force generation \cite{Charrier2020}.
\\


Intermediate filaments have been reported to be important contributors to cell contractility \cite{wu2022}.
Vimentin filaments play a role in governing actin dynamics and the transmission of contractile forces, while also influencing the alignment of cell traction stresses.
Disabling vimentin results in heightened assembly of actin stress fibers and an increase in contractility \cite{Jiu2017} \cite{patteson2022}.
Research has indicated that actomyosin contractility is necessary for the interaction between F-actin and vimentin filaments within cells on both 2D glass and in 3D cell-derived matrix \cite{Rape2011}.
The process of contractile activation leads to the phosphorylation of vimentin at Ser-56, causing a reorientation of the vimentin network. This reorientation, in turn, has been shown to enhance the transmission of contractile forces both within and among smooth muscle cells \cite{tang2019}.
The vimentin network's presence has been linked to a tenfold decrease in local actin retrograde flow rates, alongside the even distribution of actin-based forces transmitted to the substrate \cite{Nancy2019}.
\\

The cytolinker plectin plays a role in enhancing the connection between actin and vimentin.
Additionally, it engages with vimentin when subjected to forces generated by myosin contraction and the stiffness of the underlying surface.
This implies that the interaction between plectin and vimentin is responsive to mechanical cues.
It has been suggested that this mechanosensitive plectin complex hinders two-dimensional movement while being essential for propelling the nucleus forward and creating compartmentalised internal pressure within a three-dimensional cellular environment \cite{Rape2011}.
\\

While not directly a component of the contractile machinery, the microtubular network plays a role in cell contraction during the process of cell migration \cite{Costigliola2017}.
Exposing cells to either the stabilising compound taxol or the microtubule-disrupting compound nocodazole has demonstrated a reduction in both ruffling and lamellipodium formation \cite{Ballestrem2000}.
The inhibtion of microtubule polymerisation results in a broad enhancement of cell contractility and the development of stress fibers \cite{Liu1998} \cite{Liu2022}.
Hence, the overall contractile force exerted on the substrate seems to arise from a competitive interaction between the actin and microtubule cytoskeletal systems.
Actin stress fibers generate contractile force, thereby promoting the formation of focal adhesions that firmly attach them to the substrate, whereas microtubules are directed towards focal adhesions by actin fibers and contribute to their relaxation \cite{Riveline2001} \cite{Rape2011}.
\\


More recently, the role of the fourth cytokeletal compopnent septin has been shown govern the rearrangement of actin and microtubule structures while serving as a scaffold for myosin motors \cite{Spiliotis2018}.
Septins strengthen the actomyosin network by crosslinking sets of actin filaments, preparing cells for the increased mechanical requirements of migration, which involve heightened contractility.
\\

\subsection{What needs to be done?}
Although biomimetic actin networks are able to generate contractility, they have yet to fully elucidate how asymmetries in the constituent molecules contribute to these forces and the overall deformation of cells.
To understand the role of contractility in cell shape changes during migration, we envisige experiments to monitor controlled contraction-induced shape modifications in cytoskeletal GUVs.


\end{document}

==> tr.tex <==
@article{Patteson2019,
abstract = {Mammalian cells frequently migrate through tight spaces during normal embryogenesis, wound healing, diapedesis, or in pathological situations such as metastasis. Nuclear size and shape are important factors in regulating the mechanical properties of cells during their migration through such tight spaces. At the onset of migratory behavior, cells often initiate the expression of vimentin, an intermediate filament protein that polymerizes into networks extending from a juxtanuclear cage to the cell periphery. However, the role of vimentin intermediate filaments (VIFs) in regulating nuclear shape and mechanics remains unknown. Here, we use wild-type and vimentin-null mouse embryonic fibroblasts to show that VIFs regulate nuclear shape and perinuclear stiffness, cell motility in 3D, and the ability of cells to resist large deformations. These changes increase nuclear rupture and activation of DNA damage repair mechanisms, which are rescued by exogenous reexpression of vimentin. Our findings show that VIFs provide mechanical support to protect the nucleus and genome during migration.},
author = {Patteson, Alison E. and Vahabikashi, Amir and Pogoda, Katarzyna and Adam, Stephen A. and Mandal, Kalpana and Kittisopikul, Mark and Sivagurunathan, Suganya and Goldman, Anne and Goldman, Robert D. and Janmey, Paul A.},
doi = {10.1083/JCB.201902046/VIDEO-2},
issn = {15408140},
journal = {Journal of Cell Biology},
keywords = {dna damage,intermediate filaments},
mendeley-groups = {Deformability},
month = {dec},
number = {12},
pages = {4079--4092},
pmid = {31676718},
publisher = {Rockefeller University Press},
title = {{Vimentin protects cells against nuclear rupture and DNA damage during migration}},
url = {https://doi.org/10.1083/jcb.201902046},
volume = {218},
year = {2019}
}
@article{Harley2008,
abstract = {Cell migration plays a critical role in a wide variety of physiological and pathological phenomena as well as in scaffold-based tissue engineering. Cell migration behavior is known to be governed by biochemical stimuli and cellular interactions. Biophysical processes associated with interactions between the cell and its surrounding extracellular matrix may also play a significant role in regulating migration. Although biophysical properties of two-dimensional substrates have been shown to significantly influence cell migration, elucidating factors governing migration in a three-dimensional environment is a relatively new avenue of research. Here, we investigate the effect of the three-dimensional microstructure, specifically the pore size and Young's modulus, of collagen-glycosaminoglycan scaffolds on the migratory behavior of individual mouse fibroblasts. We observe that the fibroblast migration, characterized by motile fraction as well as locomotion speed, decreases as scaffold pore size increases across a range from 90 to 150 $\mu$m. Directly testing the effects of varying strut Young's modulus on cell motility showed a biphasic relationship between cell speed and strut modulus and also indicated that mechanical factors were not responsible for the observed effect of scaffold pore size on cell motility. Instead, in-depth analysis of cell locomotion paths revealed that the distribution of junction points between scaffold struts strongly modulates motility. Strut junction interactions affect local directional persistence as well as cell speed at and away from the junctions, providing a new biophysical mechanism for the governance of cell motility by the extracellular microstructure. {\textcopyright} 2008 by the Biophysical Society.},
author = {Harley, Brendan A.C. and Kim, Hyung Do and Zaman, Muhammad H. and Yannas, Ioannis V. and Lauffenburger, Douglas A. and Gibson, Lorna J.},
doi = {10.1529/BIOPHYSJ.107.122598},
file = {::},
issn = {0006-3495},
journal = {Biophysical Journal},
mendeley-groups = {Deformability},
month = {oct},
number = {8},
pages = {4013--4024},
pmid = {18621811},
publisher = {Cell Press},
title = {{Microarchitecture of Three-Dimensional Scaffolds Influences Cell Migration Behavior via Junction Interactions}},
volume = {95},
year = {2008}
}
@article{Bader2008,
abstract = {Most tissues are subject to some form of physiological mechanical loading which results in deformation of the cells triggering intracellular mechanotransduction pathways. This response to loading is generally essential for the health of the tissue, although more pronounced deformation may result in cell and tissue damage. In order to determine the biological response of cells to loading it is necessary to understand how cells and intracellular structures deform. This paper reviews the various loading systems that have been adopted for studying cell deformation both in situ within tissue explants and in isolated cell culture systems. In particular it describes loading systems which facilitate visualisation and subsequent quantification of cell deformation. The review also describes the associated microscopy and image analysis techniques. The review focuses on deformation of chondrocytes with additional information on a variety of other cell types including neurons, red blood cells, epithelial cells and skin and muscle cells. {\textcopyright} International Federation for Medical and Biological Engineering 2008.},
author = {Bader, D. L. and Knight, M. M.},
doi = {10.1007/S11517-008-0381-4/FIGURES/8},
file = {::},
issn = {01400118},
journal = {Medical and Biological Engineering and Computing},
keywords = {Biomechanics,Cell deformation,Confocal,Mechanics,Mechanotransduction},
mendeley-groups = {Deformability},
month = {aug},
number = {10},
pages = {951--963},
pmid = {18726630},
publisher = {Springer},
title = {{Biomechanical analysis of structural deformation in living cells}},
url = {https://link.springer.com/article/10.1007/s11517-008-0381-4},
volume = {46},
year = {2008}
}
@article{Lammerding2004,
abstract = {Mutations in the lamin A/C gene (LMNA) cause a variety of human diseases including Emery-Dreifuss muscular dystrophy, dilated cardiomyopathy, and Hutchinson-Gilford progeria syndrome. The tissue-specific effects of lamin mutations are unclear, in part because the function of lamin A/C is incompletely defined, but the many muscle-specific phenotypes suggest that defective lamin A/C could increase cellular mechanical sensitivity. To investigate the role of lamin A/C in mechanotransduction, we subjected lamin A/C-deficient mouse embryo fibroblasts to mechanical strain and measured nuclear mechanical properties and strain-induced signaling. We found that Lmna-/- cells have increased nuclear deformation, defective mechanotransduction, and impaired viability under mechanical strain. NF-$\kappa$B-regulated transcription in response to mechanical or cytokine stimulation was attenuated in Lmna-/- cells despite increased transcription factor binding. Lamin A/C deficiency is thus associated with both defective nuclear mechanics and impaired mechanically activated gene transcription. These findings suggest that the tissue-specific effects of lamin A/C mutations observed in the laminopathies may arise from varying degrees of impaired nuclear mechanics and transcriptional activation.},
author = {Lammerding, Jan and Schulze, P. Christian and Takahashi, Tomosaburo and Kozlov, Serguei and Sullivan, Teresa and Kamm, Roger D. and Stewart, Colin L. and Lee, Richard T.},
doi = {10.1172/JCI200419670},
file = {::},
issn = {00219738},
journal = {Journal of Clinical Investigation},
mendeley-groups = {Deformability},
month = {feb},
number = {3},
pages = {370--378},
pmid = {14755334},
title = {{Lamin A/C deficiency causes defective nuclear mechanics and mechanotransduction}},
volume = {113},
year = {2004}
}
@article{Ferrera2014,
abstract = {The architecture and structural mechanics of the cell nucleus are defined by the nuclear lamina, which is formed by A- and B-type lamins. Recently, gene duplication and protein overexpression of lamin B1 (LB1) have been reported in pedigrees with autosomal dominant leukodystrophy (ADLD). However, how the overexpression of LB1 affects nuclear mechanics and function and how it may result in pathology remain unexplored. Here, we report that in primary human skin fibroblasts derived from ADLD patients, LB1, but not other lamins, is overexpressed at the nuclear lamina and specifically enhances nuclear stiffness. Transient transfection of LB1 in HEK293 and neuronal N2a cells mimics the mechanical phenotype of ADLD nuclei. Notably, in ADLD fibroblasts, reducing LB1 protein levels by shRNA knockdown restores elasticity values to those indistinguishable from control fibroblasts. Moreover, isolated nuclei from ADLD fibroblasts display a reduced nuclear ion channel open probability on voltage-step application, suggesting that biophysical changes induced by LB1 overexpression may alter nuclear signaling cascades in somatic cells. Overall, the overexpression of LB1 in ADLD cells alters nuclear mechanics and is linked to changes in nuclear signaling, which could help explain the pathogenesis of this disease.},
author = {Ferrera, Denise and Canale, Claudio and Marotta, Roberto and Mazzaro, Nadia and Gritti, Marta and Mazzanti, Michele and Capellari, Sabina and Cortelli, Pietro and Gasparini, Laura},
doi = {10.1096/FJ.13-247635},
issn = {1530-6860},
journal = {The FASEB Journal},
keywords = {ADLD,atomic force microscopy,human fibroblasts,nuclear lamina,nucleus},
mendeley-groups = {Deformability},
month = {sep},
number = {9},
pages = {3906--3918},
pmid = {24858279},
publisher = {John Wiley & Sons, Ltd},
title = {{Lamin B1 overexpression increases nuclear rigidity in autosomal dominant leukodystrophy fibroblasts}},
url = {https://onlinelibrary.wiley.com/doi/full/10.1096/fj.13-247635 https://onlinelibrary.wiley.com/doi/abs/10.1096/fj.13-247635 https://faseb.onlinelibrary.wiley.com/doi/10.1096/fj.13-247635},
volume = {28},
year = {2014}
}
@article{Aufderhorst-Roberts2019,
abstract = {Intermediate filaments are cytoskeletal proteins that are key regulators of cell mechanics, a role which is intrinsically tied to their hierarchical structure and their unique ability to accommodate large axial strains. However, how the single-filament response to applied strains translates to networks remains unclear, particularly with regards to the crosslinking role played by the filaments' disordered “tail” domains. Here we test the role of these noncovalent crosslinks in the nonlinear rheology of reconstituted networks of the intermediate filament protein vimentin, probing their stress- and rate-dependent mechanics. Similarly to previous studies we observe elastic stress-stiffening but unlike previous work we identify a characteristic yield stress $\sigma$*, above which the networks exhibit rate-dependent softening of the network, referred to as inelastic fluidization. By investigating networks formed from tail-truncated vimentin, in which noncovalent crosslinking is suppressed, and glutaraldehyde-treated vimentin, in which crosslinking is made permanent, we show that rate-dependent inelastic fluidization is a direct consequence of vimentin's transient crosslinking. Surprisingly, although the tail–tail crosslinks are individually weak, the effective timescale for stress relaxation of the network exceeds 1000 s at $\sigma$*. Vimentin networks can therefore maintain their integrity over a large range of strains (up to ∼1000%) and loading rates (10−3 to 10−1 s−1). Our results provide insight into how the hierarchical structure of vimentin networks contributes to the cell's ability to be deformable yet strong.},
archivePrefix = {arXiv},
arxivId = {1903.10388},
author = {Aufderhorst-Roberts, Anders and Koenderink, Gijsje H.},
doi = {10.1039/C9SM00590K},
eprint = {1903.10388},
issn = {1744-6848},
journal = {Soft Matter},
mendeley-groups = {Deformability},
month = {sep},
number = {36},
pages = {7127--7136},
pmid = {31334536},
publisher = {The Royal Society of Chemistry},
title = {{Stiffening and inelastic fluidization in vimentin intermediate filament networks}},
url = {https://pubs.rsc.org/en/content/articlehtml/2019/sm/c9sm00590k https://pubs.rsc.org/en/content/articlelanding/2019/sm/c9sm00590k},
volume = {15},
year = {2019}
}
@article{Patteson2019,
abstract = {The migration of cells through constricting spaces or along fibrous tracks in tissues is important for many biological processes and depends on the mechanical properties of a cytoskeleton made up of three different filaments: F-actin, microtubules, and intermediate filaments. The signaling pathways and cytoskeletal structures that control cell motility on 2D are often very different from those that control motility in 3D. Previous studies have shown that intermediate filaments can promote actin-driven protrusions at the cell edge, but have little effect on overall motility of cells on flat surfaces. They are however important for cells to maintain resistance to repeated compressive stresses that are expected to occur in vivo. Using mouse embryonic fibroblasts derived from wild-type and vimentin-null mice, it is found that loss of vimentin increases motility in 3D microchannels even though on flat surfaces it has the opposite effect. Atomic force microscopy and traction force microscopy experiments reveal that vimentin enhances perinuclear cell stiffness while maintaining the same level of acto-myosin contractility in cells. A minimal model in which a perinuclear vimentin cage constricts along with the nucleus during motility through confining spaces, providing mechanical resistance against large strains that could damage the structural integrity of cells, is proposed.},
author = {Patteson, Alison E. and Pogoda, Katarzyna and Byfield, Fitzroy J. and Mandal, Kalpana and Ostrowska-Podhorodecka, Zofia and Charrier, Elisabeth E. and Galie, Peter A. and Deptu{\l}a, Piotr and Bucki, Robert and McCulloch, Christopher A. and Janmey, Paul A.},
doi = {10.1002/SMLL.201903180},
file = {:Users/ir.isturiz/Library/Application Support/Mendeley Desktop/Downloaded/Patteson et al. - 2019 - Loss of vimentin enhances cell motility through small confining spaces.pdf:pdf},
issn = {16136829},
journal = {Small (Weinheim an der Bergstrasse, Germany)},
keywords = {atomic force microscopy,biopolymers,constricted cell motility,traction force microscopy,vimentin},
mendeley-groups = {Deformability},
month = {dec},
number = {50},
pages = {e1903180},
pmid = {31721440},
publisher = {NIH Public Access},
title = {{Loss of vimentin enhances cell motility through small confining spaces}},
url = {/pmc/articles/PMC6910987/ /pmc/articles/PMC6910987/?report=abstract https://www.ncbi.nlm.nih.gov/pmc/articles/PMC6910987/},
volume = {15},
year = {2019}
}
@article{Zhang2023,
abstract = {Microfluidic phenotyping methods have been of vital importance for cellular characterization, especially for evaluating single cells. In order to study the deformability of a single cell, we devise...},
author = {Zhang, Ruiyun and Duan, Xuexin and Zhang, Shuaihua and Guo, Wenlan and Sun, Chen and Han, Ziyu},
doi = {10.1063/10.0017649},
file = {::},
issn = {1672-6030},
journal = {Nanotechnology and Precision Engineering},
keywords = {Cell deformation,Computer vision,Microfluidics,Single cell},
mendeley-groups = {Deformability},
month = {apr},
number = {2},
pages = {023003},
publisher = {Tianjin UniversityTianjin University},
title = {{Tunable microfluidic chip for single-cell deformation study}},
url = {https://aip.scitation.org/doi/abs/10.1063/10.0017649},
volume = {6},
year = {2023}
}
@article{Gardel2004,
abstract = {Networks of cross-linked and bundled actin filaments are ubiquitous in the cellular cytoskeleton, but their elasticity remains poorly understood. We show that these networks exhibit exceptional elastic behavior that reflects the mechanical properties of individual filaments. There are two distinct regimes of elasticity, one reflecting bending of single filaments and a second reflecting stretching of entropic fluctuations of filament length. The mechanical stiffness can vary by several decades with small changes in cross-link concentration, and can increase markedly upon application of external stress. We parameterize the full range of behavior in a state diagram and elucidate its origin with a robust model.},
author = {Gardel, M. L. and Shin, J. H. and MacKintosh, F. C. and Mahadevan, L. and Matsudaira, P. and Weitz, D. A.},
doi = {10.1126/SCIENCE.1095087/SUPPL_FILE/GARDEL.SOM.FINAL.PDF},
issn = {00368075},
journal = {Science},
mendeley-groups = {Deformability},
month = {may},
number = {5675},
pages = {1301--1305},
pmid = {15166374},
publisher = {
        American Association for the Advancement of Science
      },
title = {{Elastic behavior of cross-linked and bundled actin networks}},
url = {https://www.science.org/doi/10.1126/science.1095087},
volume = {304},
year = {2004}
}
@article{Yang2012,
abstract = {The microtubule cytoskeleton is essential in maintaining the shape, strength and organization of cells and its misregulation has been implicated in neurological disorders and cancers. To better understand the structure-mechanics relationships in microtubule networks, we measure the time- and force-dependent viscoelastic responses of entangled and sparsely crosslinked microtubule networks to precise microscale manipulation. We use magnetic tweezers devices to apply calibrated step stresses and measure the resultant strain as a function of time. At short times the material behaves as an elastic solid. The linear regime is large, with gentle stiffening observed in entangled networks above ∼70% strains. Crosslinked networks are stiffer, and show an extended linear regime. At longer times, we find a creeping regime, suggesting that structural rearrangements of the network dominate the mechanical response. To understand the molecular origins of this behaviour, we use a newly-developed portable magnetic tweezers device to observe the network morphology using a confocal microscope while simultaneously applying point-like stresses to embedded magnetic particles. We observe substantial network compression in front of the bead with no evidence of long-length scale filament flow, and find that the spatial extent of the deformation field depends sensitively on network architecture and connectivity. Our results are important to understanding the role of the cytoskeleton in regulating cargo transportin vivo, as well as the basic physics of non-affine deformations in rigid rod polymer networks.},
author = {Yang, Yali and Lin, Jun and Kaytanli, Bugra and Saleh, Omar A. and Valentine, Megan T.},
doi = {10.1039/C2SM06745E},
issn = {1744-6848},
journal = {Soft Matter},
mendeley-groups = {Deformability},
month = {jan},
number = {6},
pages = {1776--1784},
publisher = {The Royal Society of Chemistry},
title = {{Direct correlation between creep compliance and deformation in entangled and sparsely crosslinked microtubule networks}},
url = {https://pubs.rsc.org/en/content/articlehtml/2012/sm/c2sm06745e https://pubs.rsc.org/en/content/articlelanding/2012/sm/c2sm06745e},
volume = {8},
year = {2012}
}
@article{Lin2007,
abstract = {Microtubules are filamentous protein biopolymers found in eukaryotic cells. They form networks that guide active intracellular transport and support the overall cell structure. Microtubules are very rigid polymers, with persistence lengths as large as a millimeter. As such, they constitute an example of rodlike polymers, whose mechanical and rheological properties are as yet poorly understood. We measure the linear and nonlinear viscoelastic properties of isotropic solutions of purified microtubules, as well as networks permanently cross-linked with biotin-NeutrAvidin. In the linear regime both solutions and networks are soft elastic materials with elastic moduli on the order of a few pascals. The elastic moduli show a power-law dependence on tubulin concentration, c T , with G′ ∼ c T $\nu$ , where $\nu$ ≈ 1.4 for solutions and increases slightly to $\nu$ ≈ 1.6-1.8 for networks. At large deformations, we observe a concentration-dependent yield stress. The rheology of microtubule solutions cannot be explained by the Doi-Edwards model, which treats noninteracting rigid rods. Instead, they show behavior very similar to the permanently cross-linked networks, suggesting the presence of effective cross-linking even in pure microtubule solutions. We develop a simple model based on transient cross-linking interactions between microtubules to interpret the rheological response. We also calculate a lower bound estimate of the strength of this interaction. Our data provide a framework with which to understand the dynamics and mechanics of more physiological networks of microtubules with microtubule-associated cross-linking and motor proteins, and ultimately to understand the role of microtubules in cell mechanics.},
author = {Lin, Yi-Chia and Koenderink, Gijsje H and Mackintosh, Frederick C and Weitz, David A},
doi = {10.1021/ma070862l},
mendeley-groups = {Deformability},
title = {{Viscoelastic Properties of Microtubule Networks}},
year = {2007}
}
@article{VanBodegraven2020,
abstract = {Intermediate filaments (IFs), together with actin and microtubules, constitute the cytoskeleton and regulate essential biological processes including cell migration. Despite the well-described changes in the composition of IFs in migrating cells, the mechanism by which these changes may contribute to cell migration remains elusive. Recent studies show that IFs control cell migration by impacting the actomyosin machinery. This review discusses how the unique physical properties of IFs, the interplay between IFs and the actomyosin network, and the connection of IFs with cell adhesive structures participate in cell migration. We highlight the biochemical and mechanical mechanisms by which IFs control actomyosin-generated forces to influence migration speed and contribute to nuclear integrity and cell resilience to compressive forces in 2D, as well as in confined 3D migration.},
author = {van Bodegraven, Emma J. and Etienne-Manneville, Sandrine},
doi = {10.1016/J.CEB.2020.05.006},
issn = {0955-0674},
journal = {Current Opinion in Cell Biology},
keywords = {Actin,Desmosomes,Focal adhesions,Intermediate filaments,Keratin,Mechanics,Migration,Myosin,Vimentin},
mendeley-groups = {Deformability},
month = {oct},
pages = {79--88},
pmid = {32623234},
publisher = {Elsevier Current Trends},
title = {{Intermediate filaments against actomyosin: the david and goliath of cell migration}},
volume = {66},
year = {2020}
}
@article{Ribeiro2014,
abstract = {During metastasis, melanoma cells must be sufficiently deformable to squeeze through extracellular barriers with small pore sizes. We visualize and quantify deformability of single cells using micropipette aspiration and examine the migration potential of a population of melanoma cells using a flow migration apparatus. We artificially stiffen the nucleus with recombinant overexpression of $\Delta$50 lamin A, which is found in patients with Hutchison Gilford progeria syndrome and in aged individuals. Melanoma cells, both WM35 and Lu1205, both show reduced nuclear deformability and reduced cell invasion with the expression of $\Delta$50 lamin A. These studies suggest that cellular aging including expression of $\Delta$50 lamin A and nuclear stiffening may reduce the potential for metastatic cancer migration. Thus, the pathway of cancer metastasis may be kept in check by mechanical factors in addition to known chemical pathway regulation.},
author = {Ribeiro, Alexandre J.S. and Khanna, Payal and Sukumar, Aishwarya and Dong, Cheng and Dahl, Kris Noel},
doi = {10.1007/S12195-014-0358-3},
issn = {18655033},
journal = {Cellular and Molecular Bioengineering},
keywords = {Cell mechanics,Laminopathy,Metastasis},
mendeley-groups = {Deformability},
month = {dec},
number = {4},
pages = {544--551},
publisher = {Springer Science and Business Media, LLC},
title = {{Nuclear Stiffening Inhibits Migration of Invasive Melanoma Cells}},
volume = {7},
year = {2014}
}
@article{Schepers2022,
abstract = {The eukaryotic cytoskeleton consists of three different types of biopolymers - microtubules, actin filaments, and intermediate filaments - and provides cells with versatile mechanical properties, combining stability and flexibility. The unique molecular structure of intermediate filaments leads to high extensibility and stability under load. With high laser power dual optical tweezers, the mechanical properties of intermediate filaments may be investigated, while monitoring the extension with fluorescence microscopy. Here, we provide detailed protocols for the preparation of single vimentin intermediate filaments and general measurement protocols for (i) stretching experiments, (ii) repeated loading and relaxation cycles, and (iii) force-clamp experiments. We describe methods for the analysis of the experimental data in combination with computational modeling approaches.},
author = {Schepers, Anna V. and Kraxner, Julia and Lorenz, Charlotta and K{\"{o}}ster, Sarah},
doi = {10.1007/978-1-0716-2229-2_24},
issn = {1940-6029},
journal = {Methods in molecular biology (Clifton, N.J.)},
keywords = {Actin Cytoskeleton,Anna V Schepers,Cytoskeleton*,Intermediate Filaments* / chemistry,Julia Kraxner,MEDLINE,Microtubules,NCBI,NIH,NLM,National Center for Biotechnology Information,National Institutes of Health,National Library of Medicine,PubMed Abstract,Sarah K{\"{o}}ster,Vimentin / chemistry,doi:10.1007/978-1-0716-2229-2_24,pmid:36063338},
mendeley-groups = {Deformability},
pages = {677--700},
pmid = {36063338},
publisher = {Methods Mol Biol},
title = {{Mechanics of Single Vimentin Intermediate Filaments Under Load}},
url = {https://pubmed.ncbi.nlm.nih.gov/36063338/},
volume = {2478},
year = {2022}
}
@article{Lowery2015,
abstract = {Intermediate filaments (IFs) are composed of one or more members of a large family of cytoskeletal proteins, whose expression is cell- and tissue type-specific. Their importance in regulating the physiological properties of cells is becoming widely recognized in functions ranging from cell motility to signal transduction. IF proteins assemble into nanoscale biopolymers with unique strain-hardening properties that are related to their roles in regulating the mechanical integrity of cells. Furthermore, mutations in the genes encoding IF proteins cause a wide range of human diseases. Due to the number of different types of IF proteins, we have limited this short review to cover structure and function topics mainly related to the simpler homopolymeric IF networks composed of vimentin, and specifically for diseases, the related muscle-specific desmin IF networks.},
author = {Lowery, Jason and Kuczmarski, Edward R. and Herrmann, Harald and Goldma, Robert D.},
doi = {10.1074/JBC.R115.640359},
file = {::},
issn = {1083-351X},
journal = {The Journal of biological chemistry},
keywords = {Animals,Biomechanical Phenomena,Cell Movement,Cell Shape,Desmin / metabolism,Edward R Kuczmarski,Epithelial-Mesenchymal Transition,Extramural,Humans,Intermediate Filament Proteins / genetics,Intermediate Filament Proteins / metabolism,Intermediate Filaments / chemistry,Intermediate Filaments / metabolism*,Intermediate Filaments / ultrastructure,Jason Lowery,MEDLINE,Mutation,N.I.H.,NCBI,NIH,NLM,National Center for Biotechnology Information,National Institutes of Health,National Library of Medicine,Non-U.S. Gov't,Organelles / metabolism,PMC4498054,Protein Multimerization,PubMed Abstract,Research Support,Review,Robert D Goldman,Vimentin / metabolism,doi:10.1074/jbc.R115.640359,pmid:25957409},
mendeley-groups = {Deformability},
month = {jul},
number = {28},
pages = {17145--17153},
pmid = {25957409},
publisher = {J Biol Chem},
title = {{Intermediate Filaments Play a Pivotal Role in Regulating Cell Architecture and Function}},
url = {https://pubmed.ncbi.nlm.nih.gov/25957409/},
volume = {290},
year = {2015}
}
@article{Sharma2017,
abstract = {Mesenchymal stem cells (MSCs) are being studied extensively due to their potential as a therapeutic cell source for many load-bearing tissues. Compression of tissues and the subsequent deformation of cells are just one type physical strain MSCs will need to withstand in vivo. Mechanotransduction by MSCs and their mechanical properties are partially controlled by the cytoskeleton, including vimentin intermediate filaments (IFs). Vimentin IF deficiency has been tied to changes in mechanosensing and mechanical properties of cells in some cell types. However, how vimentin IFs contribute to MSC deformability has not been comprehensively studied. Investigating the role of vimentin IFs in MSC mechanosensing and mechanical properties will assist in functional understanding and development of MSC therapies. In this study, we examined vimentin IFs' contribution to MSCs' ability to deform under external deformation using RNA interference. Our results indicate that a deficient vimentin IF network decreases the deformability of MSCs, and that this may be caused by the remaining cytoskeletal network compensating for the vimentin IF network alteration. Our observations introduce another piece of information regarding how vimentin IFs are involved in the complex role the cytoskeleton plays in the mechanical properties of cells.},
author = {Sharma, Poonam and Bolten, Zachary T. and Wagner, Diane R. and Hsieh, Adam H.},
doi = {10.1007/S10439-016-1787-Z/METRICS},
issn = {15739686},
journal = {Annals of Biomedical Engineering},
keywords = {Cell deformation,Cytoskeleton,Mechanotransduction,RNA interference},
mendeley-groups = {Deformability},
month = {may},
number = {5},
pages = {1365--1374},
pmid = {28091965},
publisher = {Springer New York LLC},
title = {{Deformability of Human Mesenchymal Stem Cells Is Dependent on Vimentin Intermediate Filaments}},
url = {https://link.springer.com/article/10.1007/s10439-016-1787-z},
volume = {45},
year = {2017}
}
@article{Kasza2010,
abstract = {Networks of the cytoskeletal biopolymer actin cross-linked by the compliant protein filamin form soft gels that stiffen dramatically under shear stress. We demonstrate that the elasticity of these networks shows a strong dependence on the mean length of the actin polymers, unlike networks with small, rigid cross-links. This behavior is in agreement with a model of rigid filaments connected by multiple flexible linkers. {\textcopyright} 2010 by the Biophysical Society.},
author = {Kasza, K. E. and Broedersz, C. P. and Koenderink, G. H. and Lin, Y. C. and Messner, W. and Millman, E. A. and Nakamura, F. and Stossel, T. P. and MacKintosh, F. C. and Weitz, D. A.},
doi = {10.1016/j.bpj.2010.06.025},
file = {::},
issn = {15420086},
journal = {Biophysical Journal},
mendeley-groups = {Deformability},
month = {aug},
number = {4},
pages = {1091--1100},
publisher = {Biophysical Society},
title = {{Actin filament length tunes elasticity of flexibly cross-linked actin networks}},
url = {http://www.cell.com/article/S000634951000737X/fulltext http://www.cell.com/article/S000634951000737X/abstract https://www.cell.com/biophysj/abstract/S0006-3495(10)00737-X},
volume = {99},
year = {2010}
}
@article{Haase2015,
abstract = {Transmission of mechanical force is crucial for normal cell development and functioning. However, the process of mechanotransduction cannot be studied in isolation from cell mechanics. Thus, in order to understand how cells 'feel', we must first understand how they deform and recover from physical perturbations. Owing to its versatility, atomic force microscopy (AFM) has become a popular tool to study intrinsic cellular mechanical properties. Used to directly manipulate and examinewhole and subcellular reactions, AFM allows for topdown and reconstitutive approaches to mechanical characterization. These studies show that the responses of cells and their components are complex, and largely depend on the magnitude and time scale of loading. In this review,we generally describe themechanotransductive process through discussion of well-known mechanosensors. We then focus on discussion of recent examples where AFM is used to specifically probe the elastic and inelastic responses of single cells undergoing deformation.We present a brief overview of classical and current models often used to characterize observed cellular phenomena in response to force. Both simple mechanistic models and complex nonlinear models have been used to describe the observed cellular behaviours, however a unifying description of cell mechanics has not yet been resolved.},
author = {Haase, Kristina and Pelling, Andrew E.},
doi = {10.1098/RSIF.2014.0970},
file = {::},
issn = {17425662},
journal = {Journal of the Royal Society Interface},
keywords = {Atomic force microscopy,Cell strain,Force sensing,Mechanotransduction,Viscoelasticity},
mendeley-groups = {Deformability},
month = {mar},
number = {104},
pmid = {25589563},
publisher = {The Royal Society},
title = {{Investigating cell mechanics with atomic force microscopy}},
url = {/pmc/articles/PMC4345470/ /pmc/articles/PMC4345470/?report=abstract https://www.ncbi.nlm.nih.gov/pmc/articles/PMC4345470/},
volume = {12},
year = {2015}
}
@article{Haase2013,
abstract = {Considering that the plasma membrane is host to a variety of mechanical cues in vivo, and the actin cortex is known to support cell shape, it comes as no surprise that the paired membrane-cortex plays a major role in cellular responses to deformation. In a recent study, we applied highly localized forces to HeLa cells in order to examine the deformation response of the membrane and cortex. Direct visualization of the deformation in the loading plane allowed for the characterization of the observed time-dependent strain. Despite large magnitude and long duration loading regimes, the majority of cells recovered their initial pre-deformed morphology within $\sim$2 min. Unexpectedly, perturbed regions above large-volume nuclei were shown to be quite soft and had negligible influence on morphological recovery. The resistance to deformation and ability to recover was found to be largely influenced by the actin network, and dependent upon rho-kinase mediated contractility. {\textcopyright} 2013 Landes Bioscience.},
author = {Haase, Kristina and Pelling, Andrew E.},
doi = {10.4161/CIB.26714},
issn = {19420889},
journal = {Communicative & Integrative Biology},
keywords = {Actin,Atomic force microscopy,Cytoskeleton,Mechanotransduction,Plasma membrane},
mendeley-groups = {Deformability},
month = {nov},
number = {6},
pmid = {24349607},
publisher = {Taylor & Francis},
title = {{The role of the actin cortex in maintaining cell shape}},
url = {/pmc/articles/PMC3857327/ /pmc/articles/PMC3857327/?report=abstract https://www.ncbi.nlm.nih.gov/pmc/articles/PMC3857327/},
volume = {6},
year = {2013}
}
@article{Leduc2015,
abstract = {Cell migration is a multistep process which relies on the coordination of cytoskeletal structures in space and time. While the roles of actin and microtubules have been investigated in great details, the lack of inhibitors and visualizing tools and the large number of proteins forming intermediate filaments (IFs) have delayed the characterization of IF functions during migration. However, a large body of evidence has progressively pointed to changes in IF composition as an important parameter in the regulation of cell migratory properties both during development and tumor invasion. More recent in-depth analyses show that IFs are dynamically reorganized to participate, together with microfilaments and microtubules, to the key steps leading to cell migration.},
author = {Leduc, C{\'{e}}cile and Etienne-Manneville, Sandrine},
doi = {10.1016/J.CEB.2015.01.005},
issn = {0955-0674},
journal = {Current Opinion in Cell Biology},
mendeley-groups = {Deformability},
month = {feb},
pages = {102--112},
pmid = {25660489},
publisher = {Elsevier Current Trends},
title = {{Intermediate filaments in cell migration and invasion: the unusual suspects}},
volume = {32},
year = {2015}
}
@article{Piechocka2016,
abstract = {Bundles of polymer filaments are responsible for the rich and unique mechanical behaviors of many biomaterials, including cells and extracellular matrices. In fibrin biopolymers, whose nonlinear elastic properties are crucial for normal blood clotting, protofibrils self-assemble and bundle to form networks of semiflexible fibers. Here we show that the extraordinary strain-stiffening response of fibrin networks is a direct reflection of the hierarchical architecture of the fibrin fibers. We measure the rheology of networks of unbundled protofibrils and find excellent agreement with an affine model of extensible wormlike polymers. By direct comparison with these data, we show that physiological fibrin networks composed of thick fibers can be modeled as networks of tight protofibril bundles. We demonstrate that the tightness of coupling between protofibrils in the fibers can be tuned by the degree of enzymatic intermolecular crosslinking by the coagulation factor XIII. Furthermore, at high stress, the protofibrils contribute independently to the network elasticity, which may reflect a decoupling of the tight bundle structure. The hierarchical architecture of fibrin fibers can thus account for the nonlinearity and enormous elastic resilience characteristic of blood clots.},
author = {Piechocka, Izabela K. and Jansen, Karin A. and Broedersz, Chase P. and Kurniawan, Nicholas A. and MacKintosh, Fred C. and Koenderink, Gijsje H.},
doi = {10.1039/C5SM01992C},
file = {::},
issn = {17446848},
journal = {Soft Matter},
mendeley-groups = {Deformability},
month = {feb},
number = {7},
pages = {2145--2156},
pmid = {26761718},
publisher = {Royal Society of Chemistry},
title = {{Multi-scale strain-stiffening of semiflexible bundle networks}},
url = {https://pubs.rsc.org/en/content/articlehtml/2016/sm/c5sm01992c https://pubs.rsc.org/en/content/articlelanding/2016/sm/c5sm01992c},
volume = {12},
year = {2016}
}
@article{Urbanska2020,
abstract = {The mechanical phenotype of a cell is an inherent biophysical marker of its state and function, with many applications in basic and applied biological research. Microfluidics-based methods have enabled single-cell mechanophenotyping at throughputs comparable to those of flow cytometry. Here, we present a standardized cross-laboratory study comparing three microfluidics-based approaches for measuring cell mechanical phenotype: constriction-based deformability cytometry (cDC), shear flow deformability cytometry (sDC) and extensional flow deformability cytometry (xDC). All three methods detect cell deformability changes induced by exposure to altered osmolarity. However, a dose-dependent deformability increase upon latrunculin B-induced actin disassembly was detected only with cDC and sDC, which suggests that when exposing cells to the higher strain rate imposed by xDC, cellular components other than the actin cytoskeleton dominate the response. The direct comparison presented here furthers our understanding of the applicability of the different deformability cytometry methods and provides context for the interpretation of deformability measurements performed using different platforms. This Analysis compares microfluidics-based methods for assessing mechanical properties of cells in high throughput.},
author = {Urbanska, Marta and Mu{\~{n}}oz, Hector E. and {Shaw Bagnall}, Josephine and Otto, Oliver and Manalis, Scott R. and {Di Carlo}, Dino and Guck, Jochen},
doi = {10.1038/s41592-020-0818-8},
issn = {1548-7105},
journal = {Nature Methods 2020 17:6},
keywords = {Biophysical methods,Lab,a,chip,on},
mendeley-groups = {Deformability},
month = {apr},
number = {6},
pages = {587--593},
pmid = {32341544},
publisher = {Nature Publishing Group},
title = {{A comparison of microfluidic methods for high-throughput cell deformability measurements}},
url = {https://www.nature.com/articles/s41592-020-0818-8},
volume = {17},
year = {2020}
}
@article{McGregor2016,
abstract = {From embryonic development to cancer metastasis, cell migration plays a central role in health and disease. It is increasingly becoming apparent that cells migrating in three-dimensional (3-D) environments exhibit some striking differences compared with their well-established 2-D counterparts. One key finding is the significant role the nucleus plays during 3-D migration: when cells move in confined spaces, the cell body and nucleus must deform to squeeze through available spaces, and the deformability of the large and relatively rigid nucleus can become rate-limiting. In this review, we highlight recent findings regarding the role of nuclear mechanics in 3-D migration, including factors that govern nuclear deformability, and emerging mechanisms by which cells apply cytoskeletal forces to the nucleus to facilitate nuclear translocation. Intriguingly, the 'physical barrier' imposed by the nucleus also impacts cytoplasmic dynamics that affect cell migration and signaling, and changes in nuclear structure resulting from the mechanical forces acting on the nucleus during 3-D migration could further alter cellular function. These findings have broad relevance to the migration of both normal and cancerous cells inside living tissues, and motivate further research into the molecular details by which cells move their nuclei, as well as the consequences of the mechanical stress on the nucleus.},
author = {McGregor, Alexandra Lynn and Hsia, Chieh Ren and Lammerding, Jan},
doi = {10.1016/J.CEB.2016.01.011},
issn = {0955-0674},
journal = {Current Opinion in Cell Biology},
mendeley-groups = {Deformability},
month = {jun},
pages = {32--40},
pmid = {26895141},
publisher = {Elsevier Current Trends},
title = {{Squish and squeeze — the nucleus as a physical barrier during migration in confined environments}},
volume = {40},
year = {2016}
}
@article{Lorenz2022a,
abstract = {Different types of biological cells respond differently to mechanical stresses, and these responses are mainly governed by the cytoskeleton. The main components of this biopolymer network are actin...},
author = {Lorenz, C. and K{\"{o}}ster, S.},
doi = {10.1063/5.0099405},
file = {::},
journal = {Biophysics Reviews},
mendeley-groups = {Deformability},
month = {aug},
number = {3},
pages = {031304},
publisher = {AIP Publishing LLCAIP Publishing},
title = {{Multiscale architecture: Mechanics of composite cytoskeletal networks}},
url = {https://aip.scitation.org/doi/abs/10.1063/5.0099405},
volume = {3},
year = {2022}
}
@article{McGregor2016a,
abstract = {From embryonic development to cancer metastasis, cell migration plays a central role in health and disease. It is increasingly becoming apparent that cells migrating in three-dimensional (3-D) environments exhibit some striking differences compared with their well-established 2-D counterparts. One key finding is the significant role the nucleus plays during 3-D migration: when cells move in confined spaces, the cell body and nucleus must deform to squeeze through available spaces, and the deformability of the large and relatively rigid nucleus can become rate-limiting. In this review, we highlight recent findings regarding the role of nuclear mechanics in 3-D migration, including factors that govern nuclear deformability, and emerging mechanisms by which cells apply cytoskeletal forces to the nucleus to facilitate nuclear translocation. Intriguingly, the 'physical barrier' imposed by the nucleus also impacts cytoplasmic dynamics that affect cell migration and signaling, and changes in nuclear structure resulting from the mechanical forces acting on the nucleus during 3-D migration could further alter cellular function. These findings have broad relevance to the migration of both normal and cancerous cells inside living tissues, and motivate further research into the molecular details by which cells move their nuclei, as well as the consequences of the mechanical stress on the nucleus.},
author = {McGregor, Alexandra Lynn and Hsia, Chieh Ren and Lammerding, Jan},
doi = {10.1016/J.CEB.2016.01.011},
issn = {18790410},
journal = {Current Opinion in Cell Biology},
mendeley-groups = {Deformability},
month = {jun},
pages = {32--40},
pmid = {26895141},
publisher = {Elsevier Ltd},
title = {{Squish and squeeze - the nucleus as a physical barrier during migration in confined environments}},
volume = {40},
year = {2016}
}
@article{Castaneda2021,
abstract = {The mechanical and structural properties of actin cytoskeleton drive various cellular processes, including structural support of the plasma membrane and cellular motility. Actin monomers assemble into double-stranded helical filaments as well as higher-ordered structures such as bundles and networks. Cells incorporate macromolecular crowding, cation interactions, and actin-crosslinking proteins to regulate the organization of actin bundles. Although the roles of each of these factors in actin bundling have been well-known individually, how combined factors contribute to actin bundle assembly, organization, and mechanics is not fully understood. Here, we describe recent studies that have investigated the mechanisms of how intracellular environmental factors influence actin bundling. This review highlights the effects of macromolecular crowding, cation interactions, and actin-crosslinking proteins on actin bundle organization, structure, and mechanics. Understanding these mechanisms is important in determining in vivo actin biophysics and providing insights into cell physiology.},
author = {Castaneda, Nicholas and Park, Jinho and Kang, Ellen Hyeran},
doi = {10.3389/FPHY.2021.675885/BIBTEX},
file = {::},
issn = {2296424X},
journal = {Frontiers in Physics},
keywords = {actin bundles,actin crosslinker,bending stiffness,cation interactions,macromolecular crowding},
mendeley-groups = {Deformability},
month = {may},
pages = {227},
publisher = {Frontiers Media S.A.},
title = {{Regulation of Actin Bundle Mechanics and Structure by Intracellular Environmental Factors}},
volume = {9},
year = {2021}
}
@article{Lammerding2006,
abstract = {Mutations in the nuclear envelope proteins lamins A and C cause a broad variety of human diseases, including Emery-Dreifuss muscular dystrophy, dilated cardiomyopathy, and Hutchinson-Gilford progeria syndrome. Cells lacking lamins A and C have reduced nuclear stiffness and increased nuclear fragility, leading to increased cell death under mechanical strain and suggesting a potential mechanism for disease. Here, we investigated the contribution of major lamin subtypes (lamins A, C, and B1) to nuclear mechanics by analyzing nuclear shape, nuclear dynamics over time, nuclear deformations under strain, and cell viability under prolonged mechanical stimulation in cells lacking both lamins A and C, cells lacking only lamin A (i.e."lamin C-only" cells), cells lacking wild-type lamin B1, and wild-type cells. Lamin A/C-deficient cells exhibited increased numbers of misshapen nuclei and had severely reduced nuclear stiffness and decreased cell viability under strain. Lamin C-only cells had slightly abnormal nuclear shape and mildly reduced nuclear stiffness but no decrease in cell viability under strain. Interestingly, lamin B1-deficient cells exhibited normal nuclear mechanics despite having a significantly increased frequency of nuclear blebs. Our study indicates that lamins A and C are important contributors to the mechanical stiffness of nuclei, whereas lamin B1 contributes to nuclear integrity but not stiffness.},
author = {Lammerding, Jan and Fong, Loren G. and Ji, Julie Y. and Reue, Karen and Stewart, Colin L. and Young, Stephen G. and Lee, Richard T.},
doi = {10.1074/JBC.M513511200},
file = {::},
issn = {0021-9258},
journal = {Journal of Biological Chemistry},
mendeley-groups = {Deformability},
month = {sep},
number = {35},
pages = {25768--25780},
pmid = {16825190},
publisher = {Elsevier},
title = {{Lamins A and C but Not Lamin B1 Regulate Nuclear Mechanics}},
volume = {281},
year = {2006}
}
@article{Lin2010,
abstract = {Intermediate filament networks in the cytoplasm and nucleus are critical for the mechanical integrity of metazoan cells. However, the mechanism of crosslinking in these networks and the origins of their mechanical properties are not understood. Here, we study the elastic behavior of in vitro networks of the intermediate filament protein vimentin. Rheological experiments reveal that vimentin networks stiffen with increasing concentrations of Ca2+ and Mg2+, showing that divalent cations act as crosslinkers. We quantitatively describe the elastic response of vimentin networks over five decades of applied stress using a theory that treats the divalent cations as crosslinkers: at low stress, the behavior is entropic in origin, and increasing stress pulls out thermal fluctuations from single filaments, giving rise to a nonlinear response; at high stress, enthalpic stretching of individual filaments significantly modifies the nonlinearity. We investigate the elastic properties of networks formed by a series of protein variants with stepwise tail truncations and find that the last 11 amino acids of the C-terminal tail domain mediate crosslinking by divalent ions. We determined the single-filament persistence length, lP≈0.5 $\mu$m, and Young's modulus, Y≈9 MPa; both are consistent with literature values. Our results provide insight into a crosslinking mechanism for vimentin networks and suggest that divalent ions may help regulate the cytoskeletal structure and mechanical properties of cells. {\textcopyright} 2010 Elsevier Ltd.},
author = {Lin, Yi Chia and Broedersz, Chase P. and Rowat, Amy C. and Wedig, Tatjana and Herrmann, Harald and MacKintosh, Frederick C. and Weitz, David A.},
doi = {10.1016/J.JMB.2010.04.054},
issn = {1089-8638},
journal = {Journal of molecular biology},
keywords = {Amino Acid Sequence,Biomechanical Phenomena,Cations,Chase P Broedersz,Cross-Linking Reagents / pharmacology,David A Weitz,Divalent / pharmacology,Elastic Modulus,Electron,Humans,In Vitro Techniques,Intermediate Filaments / chemistry,Intermediate Filaments / drug effects,Intermediate Filaments / physiology,Intermediate Filaments / ultrastructure,MEDLINE,Microscopy,Molecular Sequence Data,Multiprotein Complexes / chemistry,Mutagenesis,NCBI,NIH,NLM,National Center for Biotechnology Information,National Institutes of Health,National Library of Medicine,Non-P.H.S.,Non-U.S. Gov't,Peptide Fragments / chemistry,Peptide Fragments / genetics,Peptide Fragments / physiology,Peptide Fragments / ultrastructure,Protein Structure,PubMed Abstract,Recombinant Proteins / chemistry,Recombinant Proteins / genetics,Recombinant Proteins / ultrastructure,Research Support,Rheology,Tertiary,Transmission,U.S. Gov't,Vimentin / chemistry*,Vimentin / genetics,Vimentin / physiology,Vimentin / ultrastructure,Yi-Chia Lin,doi:10.1016/j.jmb.2010.04.054,pmid:20447406},
mendeley-groups = {Deformability},
number = {4},
pages = {637--644},
pmid = {20447406},
publisher = {J Mol Biol},
title = {{Divalent cations crosslink vimentin intermediate filament tail domains to regulate network mechanics}},
url = {https://pubmed.ncbi.nlm.nih.gov/20447406/},
volume = {399},
year = {2010}
}
@article{Janmey1991,
abstract = {The mechanical properties of cytoplasm are dominated by microfilaments, microtubules, and intermediate filaments, collectively termed the cytoskeleton. This review discusses how the physical properties of these biopolymer systems are related to their molecular structures and interactions, and how remodelling of these biopolymers in vivo affects cell shape and motility. {\textcopyright} 1991.},
author = {Janmey, Paul A.},
doi = {10.1016/0955-0674(91)90159-V},
issn = {0955-0674},
journal = {Current Opinion in Cell Biology},
mendeley-groups = {Deformability},
month = {feb},
number = {1},
pages = {4--11},
pmid = {1854482},
publisher = {Elsevier Current Trends},
title = {{Mechanical properties of cytoskeletal polymers}},
volume = {3},
year = {1991}
}
@article{Shen2021,
abstract = {We investigate the rheological properties of interpenetrating networks reconstituted from the main cytoskeletal components: filamentous actin, microtubules, and vimentin intermediate filaments. The elastic modulus is determined largely by actin, with little contribution from either microtubules or vimentin. However, vimentin dramatically impacts the relaxation, with even small amounts significantly increasing the relaxation time of the interpenetrating network. This highly unusual decoupling between dissipation and elasticity may reflect weak attractive interactions between vimentin and actin networks.},
author = {Shen, Yinan and Wu, Huayin and Lu, Peter J. and Wang, Dianzhuo and Shayegan, Marjan and Li, Hui and Shi, Weichao and Wang, Zizhao and Cai, Li Heng and Xia, Jing and Zhang, Meng and Ding, Ruihua and Herrmann, Harald and Goldman, Robert and Mackintosh, Fred C. and Moncho-Jord{\'{a}}, Arturo and Weitz, David A.},
doi = {10.1103/PHYSREVLETT.127.108101/FIGURES/4/MEDIUM},
issn = {10797114},
journal = {Physical Review Letters},
mendeley-groups = {Deformability},
month = {sep},
number = {10},
pages = {108101},
pmid = {34533352},
publisher = {American Physical Society},
title = {{Effects of Vimentin Intermediate Filaments on the Structure and Dynamics of in Vitro Multicomponent Interpenetrating Cytoskeletal Networks}},
url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.127.108101},
volume = {127},
year = {2021}
}
@article{Broedersz2010,
abstract = {One of the hallmarks of biopolymer gels is their nonlinear viscoelastic response to stress, making the measurement of the mechanics of these gels very challenging. Various rheological protocols have been proposed for this; however, a thorough understanding of the techniques and their range of applicability as well as a careful comparison between these methods are still lacking. Using both strain ramp and differential prestress protocols, we investigate the nonlinear response of a variety of systems ranging from extracellular fibrin gels to intracellular F-actin solutions and F-actin cross-linked with permanent and physiological transient linkers. We find that the prestress and strain ramp results agree well for permanently cross-linked networks over two decades of strain rates, while the protocols only agree at high strain rates for more transient networks. Surprisingly, the nonlinear response measured with the prestress protocol is insensitive to creep; although a large applied steady stress can lead to significant flow, this has no significant effect on either the linear or nonlinear response of the system. A simple model is presented to provide insight into these observations.},
author = {Broedersz, Chase P. and Kasza, Karen E. and Jawerth, Louise M. and M{\"{u}}nster, Stefan and Weitz, David A. and MacKintosh, Frederick C.},
doi = {10.1039/C0SM00285B},
issn = {1744-6848},
journal = {Soft Matter},
mendeley-groups = {Deformability},
month = {aug},
number = {17},
pages = {4120--4127},
publisher = {The Royal Society of Chemistry},
title = {{Measurement of nonlinear rheology of cross-linked biopolymer gels}},
url = {https://pubs.rsc.org/en/content/articlehtml/2010/sm/c0sm00285b https://pubs.rsc.org/en/content/articlelanding/2010/sm/c0sm00285b},
volume = {6},
year = {2010}
}
@article{Wu2020,
abstract = {Divalent cations behave as effective cross-linkers of intermediate filaments (IFs) such as vimentin IF (VIF). These interactions have been mostly attributed to their multivalency. However, ion-protein interactions often depend on the ion species, and these effects have not been widely studied in IFs. Here, we investigate the effects of two biologically important divalent cations, Zn 2þ and Ca 2þ , on VIF network structure and mechanics in vitro. We find that the network structure is unperturbed at micromolar Zn 2þ concentrations, but strong bundle formation is observed at a concentration of 100 mM. Microrheological measurements show that network stiffness increases with cation concentration. However, bundling of filaments softens the network. This trend also holds for VIF networks formed in the presence of Ca 2þ , but remarkably, a concentration of Ca 2þ that is two orders higher is needed to achieve the same effect as with Zn 2þ , which suggests the importance of salt-protein interactions as described by the Hofmeister effect. Furthermore, we find evidence of competitive binding between the two divalent ion species. Hence, specific interactions between VIFs and divalent cations are likely to be an important mechanism by which cells can control their cytoplasmic mechanics.},
author = {Wu, Huayin and Shen, Yinan and Wang, Dianzhuo and Herrmann, Harald and Goldman, Robert D and Weitz, David A and Paulson, John A},
doi = {10.1016/j.bpj.2020.05.016},
mendeley-groups = {Deformability},
title = {{Effect of Divalent Cations on the Structure and Mechanics of Vimentin Intermediate Filaments}},
url = {https://doi.org/10.1016/j.bpj.2020.05.016},
year = {2020}
}
@article{Terriac2019,
abstract = {During cell spreading, cells undergo many changes to their architecture and their mechanical properties. Vimentin, as an integral part of the cell architecture, and its mechanical stability must adapt to the new state of the cell. This study focuses on the structures formed by vimentin during the first steps of cell adhesion. Very early, ball-like structures, or “knots,” are seen and often vimentin filaments emerge in the shape of rings around the nucleus. Although intermediate filaments are not known to be associated to motor proteins to form contractile systems, these rings can nonetheless strongly deform the cell nucleus. In the first 6 to 12 h of adhesion, these vimentin knots and rings disappear, and the intermediate filament network returns to the state seen before detachment of the cells. As these vimentin structures are very transient in the early steps of cell spreading, they have rarely been described in the literature. However, they can also be seen during mitosis, which is an event that involves partial detachment and re-spreading of the cells. Interestingly, the turnover dynamics of vimentin are reduced in both the knots and rings, compared to vimentin in the lamellipodia. It remains to define how the force is transmitted from the ball-like structures to the rings, and to measure the impact of such strong nuclear deformation on gene expression during cell re-spreading and the rearrangement of the vimentin network.},
author = {Terriac, Emmanuel and Sch{\"{u}}tz, Susanne and Lautenschl{\"{a}}ger, Franziska},
doi = {10.3389/FCELL.2019.00106/BIBTEX},
file = {:Users/ir.isturiz/Library/Application Support/Mendeley Desktop/Downloaded/Terriac, Sch{\"{u}}tz, Lautenschl{\"{a}}ger - 2019 - Vimentin intermediate filament rings deform the nucleus during the first steps of adhesion.pdf:pdf},
issn = {2296634X},
journal = {Frontiers in Cell and Developmental Biology},
keywords = {Adhesion,Cell spreading,Nuclear deformation,Ring,Vimentin},
mendeley-groups = {Deformability},
month = {jun},
number = {JUN},
pages = {459443},
publisher = {Frontiers Media S.A.},
title = {{Vimentin intermediate filament rings deform the nucleus during the first steps of adhesion}},
volume = {7},
year = {2019}
}
@article{Messica2017,
abstract = {Cell migration and mechanics are tightly regulated by the integrated activities of the various cytoskeletal networks. In cancer cells, cytoskeletal modulations have been implicated in the loss of tissue integrity and acquisition of an invasive phenotype. In epithelial cancers, for example, increased expression of the cytoskeletal filament protein vimentin correlates with metastatic potential. Nonetheless, the exact mechanism whereby vimentin affects cell motility remains poorly understood. In this study, we measured the effects of vimentin expression on the mechano-elastic and migratory properties of the highly invasive breast carcinoma cell line MDA231. We demonstrate here that vimentin stiffens cells and enhances cell migration in dense cultures, but exerts little or no effect on the migration of sparsely plated cells. These results suggest that cell-cell interactions play a key role in regulating cell migration, and coordinating cell movement in dense cultures. Our findings pave the way toward understanding the relationship between cell migration and mechanics in a biologically relevant context.},
author = {Messica, Yonatan and Laser-Azogui, Adi and Volberg, Tova and Elisha, Yair and Lysakovskaia, Kseniia and Eils, Roland and Gladilin, Evgeny and Geiger, Benjamin and Beck, Roy},
doi = {10.1021/ACS.NANOLETT.7B03358/SUPPL_FILE/NL7B03358_SI_004.AVI},
issn = {15306992},
journal = {Nano Letters},
keywords = {Cell motility,biophysics,cell mechanics,collective motility,metastasis,vimentin},
mendeley-groups = {Deformability},
month = {nov},
number = {11},
pages = {6941--6948},
pmid = {29022351},
publisher = {American Chemical Society},
title = {{The role of Vimentin in Regulating Cell Invasive Migration in Dense Cultures of Breast Carcinoma Cells}},
url = {https://pubs.acs.org/doi/abs/10.1021/acs.nanolett.7b03358},
volume = {17},
year = {2017}
}
@article{Fukuyama1978,
abstract = {Keratin was extracted from purified cornified cells of newborn rats in Tris-HCl-buffered 8 M urea containing /?-mercaptoethanol. Microfilaments were assembled in vitro by reducing the ionic strength of buffer and the urea concentration. One millimolar concentration of KC1 and NaCl did not affect filament formation, but the same concentration of divalent cations greatly altered this process. CaCl 2 and MgCl 2 induced gelation of keratin by formation of bundles of birefringent macrofilaments. ZnCl 2) CuSO 4 and HgCl 2 formed greater numbers of macrofilaments and the protein aggregated.},
author = {Fukuyama, Kimie and Murozuka, Takashi and Caldwell, Russell and Epstein, William L},
file = {::},
journal = {J. Cell Sci},
mendeley-groups = {Deformability},
pages = {255--263},
title = {{DIVALENT CATION STIMULATION OF IN VITRO FIBRE ASSEMBLY FROM EPIDERMAL KERATIN PROTEIN}},
volume = {33},
year = {1978}
}
@article{Schepers2021,
abstract = {The cytoskeleton, an intricate network of protein filaments, motor proteins, and cross-linkers, largely determines the mechanical properties of cells. Among the three filamentous components, F-actin, microtubules, and intermediate filaments (IFs), the IF network is by far the most extensible and resilient to stress. We present a multiscale approach to disentangle the three main contributions to vimentin IF network mechanics-single-filament mechanics, filament length, and interactions between filaments-including their temporal evolution. Combining particle tracking, quadruple optical trapping, and computational modeling, we derive quantitative information on the strength and kinetics of filament interactions. Specifically, we find that hydrophobic contributions to network mechanics enter mostly via filament-elongation kinetics, whereas electrostatics have a direct influence on filament-filament interactions.},
author = {Schepers, Anna V. and Lorenz, Charlotta and Nietmann, Peter and Janshoff, Andreas and Klumpp, Stefan and K{\"{o}}ster, Sarah},
doi = {10.1073/PNAS.2102026118/-/DCSUPPLEMENTAL},
file = {::},
issn = {10916490},
journal = {Proceedings of the National Academy of Sciences of the United States of America},
keywords = {Cytoskeleton,Intermediate filaments,Microrheology,Network mechanics,Quadruple optical tweezers},
mendeley-groups = {Deformability},
month = {jul},
number = {27},
pmid = {34187892},
publisher = {National Academy of Sciences},
title = {{Multiscale mechanics and temporal evolution of vimentin intermediate filament networks}},
url = {https://pubmed.ncbi.nlm.nih.gov/34187892/},
volume = {118},
year = {2021}
}
@article{Seltmann2013,
abstract = {Cell motility and cell shape adaptations are crucial during wound healing, inflammation, and malignant progression. These processes require the remodeling of the keratin cytoskeleton to facilitate cell-cell and cell-matrix adhesion. However, the role of keratins for biomechanical properties and invasion of epithelial cells is only partially understood. In this study, we address this issue in murine keratinocytes lacking all keratins on genome engineering. In contrast to predictions, keratin-free cells show about 60% higher cell deformability even for small deformations. This response is compared with the less pronounced softening effects for actin depolymerization induced via latrunculin A. To relate these findings with functional consequences, we use invasion and 3D growth assays. These experiments reveal higher invasiveness of keratin-free cells. Reexpression of a small amount of the keratin pair K5/K14 in keratin-free cells reverses the above phenotype for the invasion but does not with respect to cell deformability. Our data show a unique role of keratins as major players of cell stiffness, influencing invasion with implications for epidermal homeostasis and pathogenesis. This study supports the view that down-regulation of keratins observed during epithelial-mesenchymal transition directly contributes to the migratory and invasive behavior of tumor cells.},
author = {Seltmann, Kristin and Fritsch, Anatol W. and K{\"{a}}s, Josef A. and Magin, Thomas M.},
doi = {10.1073/PNAS.1310493110/-/DCSUPPLEMENTAL},
file = {::},
issn = {00278424},
journal = {Proceedings of the National Academy of Sciences of the United States of America},
keywords = {Boyden chamber,Cell mechanics,Intermediate filaments,Optical stretcher},
mendeley-groups = {Deformability},
month = {nov},
number = {46},
pages = {18507--18512},
pmid = {24167274},
publisher = {National Academy of Sciences},
title = {{Keratins significantly contribute to cell stiffness and impact invasive behavior}},
url = {/pmc/articles/PMC3832002/ /pmc/articles/PMC3832002/?report=abstract https://www.ncbi.nlm.nih.gov/pmc/articles/PMC3832002/},
volume = {110},
year = {2013}
}
@article{Janmey1991a,
abstract = {The cytoplasm of vertebrate cells contains three distinct filamentous biopolymers, the microtubules, microfilaments, and intermediate filaments. The basic structural elements of these three filaments are linear polymers of the proteins tubulin, actin, and vimentin or another related intermediate filament protein, respectively. The viscoelastic properties of cytoplasmic filaments are likely to be relevant to their biologic function, because their extreme length and rodlike structure dominate the rheologic behavior of cytoplasm, and changes in their structure may cause gel-sol transitions observed when cells are activated or begin to move. This paper describes parallel measurements of the viscoelasticity of tubulin, actin, and vimentin polymers. The rheologic differences among the three types of cytoplasmic polymers suggest possible specialized roles for the different classes of filaments in vivo. Actin forms networks of highest rigidity that fluidize at high strains, consistent with a role in cell motility in which stable protrusions can deform rapidly in response to controlled filament rupture. Vimentin networks, which have not previously been studied by rheologic methods, exhibit some unusual viscoelastic properties not shared by actin or tubulin. They are less rigid (have lower shear moduli) at low strain but harden at high strains and resist breakage, suggesting they maintain cell integrity. The differences between F-actin and vimentin are optimal for the formation of a composite material with a range of properties that cannot be achieved by either polymer alone. Microtubules are unlikely to contribute significantly to interphase cell rheology alone, but may help stabilize the other networks.},
author = {Janmey, P. A. and Euteneuer, U. and Traub, P. and Schliwa, M.},
doi = {10.1083/JCB.113.1.155},
issn = {00219525},
journal = {The Journal of Cell Biology},
mendeley-groups = {Deformability},
month = {apr},
number = {1},
pages = {155},
pmid = {2007620},
publisher = {The Rockefeller University Press},
title = {{Viscoelastic properties of vimentin compared with other filamentous biopolymer networks}},
url = {/pmc/articles/PMC2288924/?report=abstract https://www.ncbi.nlm.nih.gov/pmc/articles/PMC2288924/},
volume = {113},
year = {1991}
}
@article{Schaedel2021,
abstract = {The cytoskeleton determines cell mechanics and lies at the heart of important cellular functions. Growing evidence suggests that the manifold tasks of the cytoskeleton rely on the interactions between its filamentous components—actin filaments, intermediate filaments, and microtubules. However, the nature of these interactions and their impact on cytoskeletal dynamics are largely unknown. Here, we show in a reconstituted in vitro system that vimentin intermediate filaments stabilize microtubules against depolymerization and support microtubule rescue. To understand these stabilizing effects, we directly measure the interaction forces between individual microtubules and vimentin filaments. Combined with numerical simulations, our observations provide detailed insight into the physical nature of the interactions and how they affect microtubule dynamics. Thus, we describe an additional, direct mechanism by which cells establish the fundamental cross talk of cytoskeletal components alongside linker proteins. Moreover, we suggest a strategy to estimate the binding energy of tubulin dimers within the microtubule lattice. The tasks of the cytoskeleton depend on the fine-tuned interplay between the three filamentous components: actin filaments, microtubules, and intermediate filaments. Here, the authors show in a reconstituted in vitro system that vimentin intermediate filaments stabilize microtubules against depolymerization and support microtubule rescue by direct interactions.},
author = {Schaedel, Laura and Lorenz, Charlotta and Schepers, Anna V. and Klumpp, Stefan and K{\"{o}}ster, Sarah},
doi = {10.1038/s41467-021-23523-z},
file = {::},
issn = {2041-1723},
journal = {Nature Communications 2021 12:1},
keywords = {Biological physics,Biophysics},
mendeley-groups = {Deformability},
month = {jun},
number = {1},
pages = {1--12},
pmid = {34145230},
publisher = {Nature Publishing Group},
title = {{Vimentin intermediate filaments stabilize dynamic microtubules by direct interactions}},
url = {https://www.nature.com/articles/s41467-021-23523-z},
volume = {12},
year = {2021}
}
@article{Schaedel2021,
abstract = {The cytoskeleton determines cell mechanics and lies at the heart of important cellular functions. Growing evidence suggests that the manifold tasks of the cytoskeleton rely on the interactions between its filamentous components—actin filaments, intermediate filaments, and microtubules. However, the nature of these interactions and their impact on cytoskeletal dynamics are largely unknown. Here, we show in a reconstituted in vitro system that vimentin intermediate filaments stabilize microtubules against depolymerization and support microtubule rescue. To understand these stabilizing effects, we directly measure the interaction forces between individual microtubules and vimentin filaments. Combined with numerical simulations, our observations provide detailed insight into the physical nature of the interactions and how they affect microtubule dynamics. Thus, we describe an additional, direct mechanism by which cells establish the fundamental cross talk of cytoskeletal components alongside linker proteins. Moreover, we suggest a strategy to estimate the binding energy of tubulin dimers within the microtubule lattice. The tasks of the cytoskeleton depend on the fine-tuned interplay between the three filamentous components: actin filaments, microtubules, and intermediate filaments. Here, the authors show in a reconstituted in vitro system that vimentin intermediate filaments stabilize microtubules against depolymerization and support microtubule rescue by direct interactions.},
author = {Schaedel, Laura and Lorenz, Charlotta and Schepers, Anna V. and Klumpp, Stefan and K{\"{o}}ster, Sarah},
doi = {10.1038/s41467-021-23523-z},
file = {::},
issn = {2041-1723},
journal = {Nature Communications 2021 12:1},
keywords = {Biological physics,Biophysics},
mendeley-groups = {Deformability},
month = {jun},
number = {1},
pages = {1--12},
pmid = {34145230},
publisher = {Nature Publishing Group},
title = {{Vimentin intermediate filaments stabilize dynamic microtubules by direct interactions}},
url = {https://www.nature.com/articles/s41467-021-23523-z},
volume = {12},
year = {2021}
}
@article{Wagner2007,
abstract = {One cellular function of intermediate filaments is to provide cells with compliance to small deformations while strengthening them when large stresses are applied. How IFs accomplish this mechanical role is revealed by recent studies of the elastic properties of single IF protein polymers and by viscoelastic characterization of the networks they form. IFs are unique among cytoskeletal filaments in withstanding large deformations. Single filaments can stretch to more than 3 times their initial length before breaking, and gels of IF withstand strains greater than 100% without damage. Even after mechanical disruption of gels formed by crossbridged neurofilaments, the elastic modulus of these gels rapidly recovers under conditions where gels formed by actin filaments are irreversibly ruptured. The polyelectrolyte properties of IFs may enable crossbridging by multivalent counterions, but identifying the mechanisms by which IFs link into bundles and networks in vivo remains a challenge. {\textcopyright} 2007 Elsevier Inc. All rights reserved.},
author = {Wagner, Oliver I. and Rammensee, Sebastian and Korde, Neha and Wen, Qi and Leterrier, Jean Francois and Janmey, Paul A.},
doi = {10.1016/J.YEXCR.2007.04.025},
file = {::},
issn = {00144827},
journal = {Experimental cell research},
keywords = {Elasticity,Network,Neurofilament,Polyelectrolyte,Viscoelasticity},
mendeley-groups = {Deformability},
month = {jun},
number = {10},
pages = {2228},
pmid = {17524395},
publisher = {NIH Public Access},
title = {{Softness, strength and self-repair in intermediate filament networks}},
url = {/pmc/articles/PMC2709732/ /pmc/articles/PMC2709732/?report=abstract https://www.ncbi.nlm.nih.gov/pmc/articles/PMC2709732/},
volume = {313},
year = {2007}
}
@article{Kreplak2005,
abstract = {Intermediate filaments (IFs) are structural elements of eukaryotic cells with distinct mechanical properties. Tissue integrity is severely impaired, in particular in skin and muscle, when IFs are either absent or malfunctioning due to mutations. Our knowledge on the mechanical properties of IFs is mainly based on tensile testing of macroscopic fibers and on the rheology of IF networks. At the single filament level, the only piece of data available is a measure of the persistence length of vimentin IFs. Here, we have employed an atomic force microscopy (AFM) based protocol to directly probe the mechanical properties of single cytoplasmic IFs when adsorbed to a solid support in physiological buffer environment. Three IF types were studied in vitro: recombinant murine desmin, recombinant human keratin K5/K14 and neurofilaments isolated from rat brains, which are composed of the neurofilament triplet proteins NF-L, NF-M and NF-H. Depending on the experimental conditions, the AFM tip was used to laterally displace or to stretch single IFs on the support they had been adsorbed to. Upon applying force, IFs were stretched on average 2.6-fold. The maximum stretching that we encountered was 3.6-fold. A large reduction of the apparent filament diameter was observed concomitantly. The observed mechanical properties therefore suggest that IFs may indeed function as mechanical shock absorbers in vivo. {\textcopyright} 2005 Elsevier Ltd. All rights reserved.},
author = {Kreplak, L. and B{\"{a}}r, H. and Leterrier, J. F. and Herrmann, H. and Aebi, U.},
doi = {10.1016/J.JMB.2005.09.092},
issn = {0022-2836},
journal = {Journal of molecular biology},
keywords = {Animals,Atomic Force,Desmin / chemistry,Desmin / ultrastructure,H B{\"{a}}r,Humans,Intermediate Filaments / chemistry,Intermediate Filaments / metabolism*,Intermediate Filaments / ultrastructure*,Keratins / chemistry,Keratins / ultrastructure,L Kreplak,MEDLINE,Mice,Microscopy,NCBI,NIH,NLM,Nanotechnology,National Center for Biotechnology Information,National Institutes of Health,National Library of Medicine,Neurofilament Proteins / chemistry,Neurofilament Proteins / ultrastructure,Non-U.S. Gov't,PubMed Abstract,Rats,Research Support,Time Factors,U Aebi,doi:10.1016/j.jmb.2005.09.092,pmid:16257415},
mendeley-groups = {Deformability},
month = {dec},
number = {3},
pages = {569--577},
pmid = {16257415},
publisher = {J Mol Biol},
title = {{Exploring the mechanical behavior of single intermediate filaments}},
url = {https://pubmed.ncbi.nlm.nih.gov/16257415/},
volume = {354},
year = {2005}
}
@article{Lin2010,
abstract = {Intermediate filaments are common structural elements found in abundance in all metazoan cells, where they form networks that contribute to the elasticity. Here, we report measurements of the linear and nonlinear viscoelasticity of networks of two distinct intermediate filaments, vimentin and neurofilaments. Both exhibit predominantly elastic behavior with strong nonlinear strain stiffening. We demonstrate that divalent ions behave as effective cross-linkers for both networks, and that the elasticity of these networks is consistent with the theory for that of semiflexible polymers. {\textcopyright} 2010 The American Physical Society.},
author = {Lin, Yi Chia and Yao, Norman Y. and Broedersz, Chase P. and Herrmann, Harald and MacKintosh, Fred C. and Weitz, David A.},
doi = {10.1103/PHYSREVLETT.104.058101},
issn = {1079-7114},
journal = {Physical review letters},
keywords = {Animals,Cattle,David A Weitz,Elasticity*,Humans,Intermediate Filaments / chemistry*,MEDLINE,NCBI,NIH,NLM,National Center for Biotechnology Information,National Institutes of Health,National Library of Medicine,Non-P.H.S.,Non-U.S. Gov't,Norman Y Yao,PubMed Abstract,Research Support,U.S. Gov't,Vimentin / chemistry,Yi-Chia Lin,doi:10.1103/PhysRevLett.104.058101,pmid:20366795},
mendeley-groups = {Deformability},
month = {feb},
number = {5},
pmid = {20366795},
publisher = {Phys Rev Lett},
title = {{Origins of elasticity in intermediate filament networks}},
url = {https://pubmed.ncbi.nlm.nih.gov/20366795/},
volume = {104},
year = {2010}
}
@article{Wu2020,
abstract = {Divalent cations behave as effective cross-linkers of intermediate filaments (IFs) such as vimentin IF (VIF). These interactions have been mostly attributed to their multivalency. However, ion-protein interactions often depend on the ion species, and these effects have not been widely studied in IFs. Here, we investigate the effects of two biologically important divalent cations, Zn2+ and Ca2+, on VIF network structure and mechanics in vitro. We find that the network structure is unperturbed at micromolar Zn2+ concentrations, but strong bundle formation is observed at a concentration of 100 $\mu$M. Microrheological measurements show that network stiffness increases with cation concentration. However, bundling of filaments softens the network. This trend also holds for VIF networks formed in the presence of Ca2+, but remarkably, a concentration of Ca2+ that is two orders higher is needed to achieve the same effect as with Zn2+, which suggests the importance of salt-protein interactions as described by the Hofmeister effect. Furthermore, we find evidence of competitive binding between the two divalent ion species. Hence, specific interactions between VIFs and divalent cations are likely to be an important mechanism by which cells can control their cytoplasmic mechanics.},
author = {Wu, Huayin and Shen, Yinan and Wang, Dianzhuo and Herrmann, Harald and Goldman, Robert D. and Weitz, David A.},
doi = {10.1016/J.BPJ.2020.05.016},
file = {::},
issn = {15420086},
journal = {Biophysical Journal},
mendeley-groups = {Deformability},
month = {jul},
number = {1},
pages = {55},
pmid = {32521238},
publisher = {The Biophysical Society},
title = {{Effect of Divalent Cations on the Structure and Mechanics of Vimentin Intermediate Filaments}},
url = {/pmc/articles/PMC7335910/ /pmc/articles/PMC7335910/?report=abstract https://www.ncbi.nlm.nih.gov/pmc/articles/PMC7335910/},
volume = {119},
year = {2020}
}
@article{Yao2010,
abstract = {Neurofilaments are found in abundance in the cytoskeleton of neurons, where they act as an intracellular framework protecting the neuron from external stresses. To elucidate the nature of the mechanical properties that provide this protection, we measure the linear and nonlinear viscoelastic properties of networks of neurofilaments. These networks are soft solids that exhibit dramatic strain stiffening above critical strains of 30-70%. Surprisingly, divalent ions such as Mg2+, Ca2+, and Zn2+ act as effective cross-linkers for neurofilament networks, controlling their solidlike elastic response. This behavior is comparable to that of actin-binding proteins in reconstituted filamentous actin. We show that the elasticity of neurofilament networks is entropic in origin and is consistent with a model for cross-linked semiflexible networks, which we use to quantify the cross-linking by divalent ions. {\textcopyright} 2010 by the Biophysical Society.},
author = {Yao, Norman Y. and Braedersz, Chase P. and Lin, Yi Chia and Kasza, Karen E. and MacKintosh, Frederick C. and Weitz, David A.},
doi = {10.1016/j.bpj.2010.01.062},
file = {::},
issn = {15420086},
journal = {Biophysical Journal},
mendeley-groups = {Deformability},
month = {may},
number = {10},
pages = {2147--2153},
pmid = {20483322},
publisher = {Biophysical Society},
title = {{Elasticity in lonically cross-linked neurofilament networks}},
url = {http://www.cell.com/article/S0006349510002304/fulltext http://www.cell.com/article/S0006349510002304/abstract https://www.cell.com/biophysj/abstract/S0006-3495(10)00230-4},
volume = {98},
year = {2010}
}
@article{Golde2018,
abstract = {The cytoskeleton is a highly interconnected meshwork of strongly coupled subsystems providing mechanical stability as well as dynamic functions to cells. To elucidate the underlying biophysical principles, it is central to investigate not only one distinct functional subsystem but rather their interplay as composite biopolymeric structures. Two of the key cytoskeletal elements are actin and vimentin filaments. Here, we show that composite networks reconstituted from actin and vimentin can be described by a superposition of two non-interacting scaffolds. Arising effects are demonstrated in a scale-spanning frame connecting single filament dynamics to macro-rheological network properties. The acquired results of the linear and non-linear bulk mechanics can be captured within an inelastic glassy wormlike chain model. In contrast to previous studies, we find no emergent effects in these composite networks. Thus, our study paves the way to predict the mechanics of the cytoskeleton based on the properties of its single structural components.},
author = {Golde, Tom and Huster, Constantin and Glaser, Martin and H{\"{a}}ndler, Tina and Herrmann, Harald and K{\"{a}}s, Josef A. and Schnau{\ss}, J{\"{o}}rg},
doi = {10.1039/C8SM01061G},
file = {::},
issn = {17446848},
journal = {Soft Matter},
mendeley-groups = {Deformability},
number = {39},
pages = {7970--7978},
pmid = {30176034},
publisher = {Royal Society of Chemistry},
title = {{Glassy dynamics in composite biopolymer networks}},
volume = {14},
year = {2018}
}
@article{Esue2006,
abstract = {The assembly and organization of the three major eukaryotic cytoskeleton proteins, actin, microtubules, and intermediate filaments, are highly interdependent. Through evolution, cells have developed specialized multifunctional proteins that mediate the cross-linking of these cytoskeleton filament networks. Here we test the hypothesis that two of these filamentous proteins, F-actin and vimentin filament, can interact directly, i.e. in the absence of auxiliary proteins. Through quantitative rheological studies, we find that a mixture of vimentin/actin filament network features a significantly higher stiffness than that of networks containing only actin filaments or only vimentin filaments. Maximum inter-filament interaction occurs at a vimentin/ actin molar ratio of 3 to 1. Mixed networks of actin and tailless vimentin filaments show low mechanical stiffness and much weaker inter-filament interactions. Together with the fact that cells featuring prominent vimentin and actin networks are much stiffer than their counterparts lacking an organized actin or vimentin network, these results suggest that actin and vimentin filaments can interact directly through the tail domain of vimentin and that these inter-filament interactions may contribute to the overall mechanical integrity of cells and mediate cytoskeletal cross-talk. {\textcopyright} 2006 by The American Society for Biochemistry and Molecular Biology, Inc.},
author = {Esue, Osigwe and Carson, Ashley A. and Tseng, Yiider and Wirtz, Denis},
doi = {10.1074/JBC.M605452200},
file = {::},
issn = {0021-9258},
journal = {The Journal of biological chemistry},
keywords = {Actins / chemistry*,Animals,Ashley A Carson,Chickens,Cytoskeleton / metabolism,Denis Wirtz,Dose-Response Relationship,Drug,Extramural,Humans,Kinetics,MEDLINE,Microtubules / metabolism,N.I.H.,NCBI,NIH,NLM,National Center for Biotechnology Information,National Institutes of Health,National Library of Medicine,Non-P.H.S.,Non-U.S. Gov't,Osigwe Esue,Protein Binding,Protein Structure,PubMed Abstract,Research Support,Tertiary,U.S. Gov't,Vimentin / chemistry*,doi:10.1074/jbc.M605452200,pmid:16901892},
mendeley-groups = {Deformability},
month = {oct},
number = {41},
pages = {30393--30399},
pmid = {16901892},
publisher = {J Biol Chem},
title = {{A direct interaction between actin and vimentin filaments mediated by the tail domain of vimentin}},
url = {https://pubmed.ncbi.nlm.nih.gov/16901892/},
volume = {281},
year = {2006}
}
@article{Lin2007,
abstract = {Microtubules are filamentous protein biopolymers found in eukaryotic cells. They form networks that guide active intracellular transport and support the overall cell structure. Microtubules are very rigid polymers, with persistence lengths as large as a millimeter. As such, they constitute an example of rodlike polymers, whose mechanical and rheological properties are as yet poorly understood. We measure the linear and nonlinear viscoelastic properties of isotropic solutions of purified microtubules, as well as networks permanently cross-linked with biotin-NeutrAvidin. In the linear regime both solutions and networks are soft elastic materials with elastic moduli on the order of a few pascals. The elastic moduli show a power-law dependence on tubulin concentration, c T, with G′ ∼ c Tv, where v ≈1.4 for solutions and increases slightly to v ≈1.6-1.8 for networks. At large deformations, we observe a concentration-dependent yield stress. The rheology of microtubule solutions cannot be explained by the Doi-Edwards model, which treats noninteracting rigid rods. Instead, they show behavior very similar to the permanently cross-linked networks, suggesting the presence of effective cross-linking even in pure microtubule solutions. We develop a simple model based on transient cross-linking interactions between microtubules to interpret the rheological response. We also calculate a lower bound estimate of the strength of this interaction. Our data provide a framework with which to understand the dynamics and mechanics of more physiological networks of microtubules with microtubule-associated cross-linking and motor proteins, and ultimately to understand the role of microtubules in cell mechanics. {\textcopyright} 2007 American Chemical Society.},
author = {Lin, Yi Chia and Koenderink, Gijsje H. and MacKintosh, Frederick C. and Weitz, David A.},
doi = {10.1021/MA070862L/ASSET/IMAGES/MEDIUM/MA070862LN00001.GIF},
issn = {00249297},
journal = {Macromolecules},
mendeley-groups = {Deformability},
month = {oct},
number = {21},
pages = {7714--7720},
publisher = { American Chemical Society },
title = {{Viscoelastic properties of microtubule networks}},
url = {https://pubs.acs.org/doi/pdf/10.1021/ma070862l},
volume = {40},
year = {2007}
}
@article{Kasza2010,
abstract = {Networks of the cytoskeletal biopolymer actin cross-linked by the compliant protein filamin form soft gels that stiffen dramatically under shear stress. We demonstrate that the elasticity of these networks shows a strong dependence on the mean length of the actin polymers, unlike networks with small, rigid cross-links. This behavior is in agreement with a model of rigid filaments connected by multiple flexible linkers. {\textcopyright} 2010 by the Biophysical Society.},
author = {Kasza, K. E. and Broedersz, C. P. and Koenderink, G. H. and Lin, Y. C. and Messner, W. and Millman, E. A. and Nakamura, F. and Stossel, T. P. and MacKintosh, F. C. and Weitz, D. A.},
doi = {10.1016/J.BPJ.2010.06.025},
file = {::},
issn = {15420086},
journal = {Biophysical Journal},
mendeley-groups = {Deformability},
month = {aug},
number = {4},
pages = {1091},
pmid = {20712992},
publisher = {The Biophysical Society},
title = {{Actin Filament Length Tunes Elasticity of Flexibly Cross-Linked Actin Networks}},
url = {/pmc/articles/PMC2920742/ /pmc/articles/PMC2920742/?report=abstract https://www.ncbi.nlm.nih.gov/pmc/articles/PMC2920742/},
volume = {99},
year = {2010}
}
@article{Block2018,
abstract = {Structure and dynamics of living matter rely on design principles fundamentally different from concepts of traditional material science. Specialized intracellular filaments in the cytoskeleton permit living systems to divide, migrate, and grow with a high degree of variability and durability. Among the three filament systems, microfilaments, microtubules, and intermediate filaments (IFs), the physical properties of IFs and their role in cellular mechanics are the least well understood. We use optical trapping of individual vimentin filaments to investigate energy dissipation, strain history dependence, and creep behavior of stretched filaments. By stochastic and numerical modeling, we link our experimental observations to the peculiar molecular architecture of IFs. We find that individual vimentin filaments display tensile memory and are able to dissipate more than 70% of the input energy. We attribute these phenomena to distinct nonequilibrium folding and unfolding of a helices in the vimentin monomers constituting the filaments.},
author = {Block, Johanna and Witt, Hannes and Candelli, Andrea and Danes, Jordi Cabanas and Peterman, Erwin J.G. and Wuite, Gijs J.L. and Janshoff, Andreas and K{\"{o}}ster, Sarah},
doi = {10.1126/SCIADV.AAT1161/SUPPL_FILE/AAT1161_SM.PDF},
file = {::},
issn = {23752548},
journal = {Science Advances},
mendeley-groups = {Deformability},
month = {jun},
number = {6},
pmid = {29928696},
publisher = {American Association for the Advancement of Science},
title = {{Viscoelastic properties of vimentin originate from nonequilibrium conformational changes}},
url = {https://www.science.org/doi/10.1126/sciadv.aat1161},
volume = {4},
year = {2018}
}
@article{VanMameren2009,
abstract = {The micrometer-scale length of some protein polymers allows them to be mechanically manipulated in singlemolecule experiments. This provides a direct way to measure persistence length. We have used a double optical trap to elastically deform single microtubules and actin filaments. Axial extensional force was exerted on beads attached laterally to the filaments. Because the attachments are off the line of force, pulling the beads apart couples to local bending of the filament. We present a simple mechanical model for the resulting highly nonlinear elastic response of the dumbbell construct. The flexural rigidities of the microfilaments that were found by fitting the model to the experimentally observed force-distance curves are (7.1 ± 0.8) × 104 pN{\textperiodcentered}nm2 (persistence length L p = 17.2 $\mu$ m) for F-actin and (6.1 ± 1.3) × 106 pN{\textperiodcentered}nm2 ( L p = 1.4 mm) for microtubules. {\textcopyright} 2009 American Chemical Society.},
author = {{Van Mameren}, Joost and Vermeulen, Karen C. and Gittes, Fred and Schmidt, Christoph F.},
doi = {10.1021/JP808328A},
issn = {1520-6106},
journal = {The journal of physical chemistry. B},
keywords = {Actins / chemistry*,Animals,Chemical,Christoph F Schmidt,Elasticity,Joost van Mameren,Karen C Vermeulen,MEDLINE,Models,NCBI,NIH,NLM,National Center for Biotechnology Information,National Institutes of Health,National Library of Medicine,Non-U.S. Gov't,Polymers / chemistry*,PubMed Abstract,Research Support,Shear Strength,Swine,Tubulin / chemistry,doi:10.1021/jp808328a,pmid:19673071},
mendeley-groups = {Deformability},
month = {mar},
number = {12},
pages = {3837--3844},
pmid = {19673071},
publisher = {J Phys Chem B},
title = {{Leveraging single protein polymers to measure flexural rigidity}},
url = {https://pubmed.ncbi.nlm.nih.gov/19673071/},
volume = {113},
year = {2009}
}
@article{Wolf2013,
abstract = {Cell migration through 3D tissue depends on a physicochemical balance between cell deformability and physical tissue constraints. Migration rates are further governed by the capacity to degrade ECM by proteolytic enzymes, particularly matrix metalloproteinases (MMPs), and integrin- and actomyosin-mediated mechanocoupling. Yet, how these parameters cooperate when space is confined remains unclear. Using MMPdegradable collagen lattices or nondegradable substrates of varying porosity, we quantitatively identify the limits of cell migration by physical arrest. MMP-independent migration declined as linear function of pore size and with deformation of the nucleus, with arrest reached at 10% of the nuclear cross section (tumor cells, 7 $\mu$m2; T cells, 4 $\mu$m2; neutrophils, 2 $\mu$m2). Residual migration under space restriction strongly depended upon MMPdependent ECM cleavage by enlarging matrix pore diameters, and integrin- and actomyosin-dependent force generation, which jointly propelled the nucleus. The limits of interstitial cell migration thus depend upon scaffold porosity and deformation of the nucleus, with pericellular collagenolysis and mechanocoupling as modulators. {\textcopyright} 2013 Wolf et al.},
author = {Wolf, Katarina and te Lindert, Mariska and Krause, Marina and Alexander, Stephanie and te Riet, Joost and Willis, Amanda L. and Hoffman, Robert M. and Figdor, Carl G. and Weiss, Stephen J. and Friedl, Peter},
doi = {10.1083/JCB.201210152},
file = {::},
issn = {1540-8140},
journal = {The Journal of cell biology},
keywords = {Animals,Cattle,Cell Line,Cell Movement / physiology*,Collagen / chemistry,Extracellular Matrix / physiology*,Extracellular Matrix / ultrastructure,Extramural,Humans,Hydrogels / chemistry,Integrins / metabolism,Katarina Wolf,Kinetics,MEDLINE,Mariska Te Lindert,Matrix Metalloproteinases / metabolism,Matrix Metalloproteinases / physiology,N.I.H.,NCBI,NIH,NLM,National Center for Biotechnology Information,National Institutes of Health,National Library of Medicine,Non-U.S. Gov't,PMC3691458,Peter Friedl,Proteolysis,PubMed Abstract,Rats,Research Support,Surface Properties,doi:10.1083/jcb.201210152,pmid:23798731},
mendeley-groups = {Deformability},
month = {jun},
number = {7},
pages = {1069--1084},
pmid = {23798731},
publisher = {J Cell Biol},
title = {{Physical limits of cell migration: control by ECM space and nuclear deformation and tuning by proteolysis and traction force}},
url = {https://pubmed.ncbi.nlm.nih.gov/23798731/},
volume = {201},
year = {2013}
}
@article{McGregor2016,
abstract = {From embryonic development to cancer metastasis, cell migration plays a central role in health and disease. It is increasingly becoming apparent that cells migrating in three-dimensional (3-D) environments exhibit some striking differences compared with their well-established 2-D counterparts. One key finding is the significant role the nucleus plays during 3-D migration: when cells move in confined spaces, the cell body and nucleus must deform to squeeze through available spaces, and the deformability of the large and relatively rigid nucleus can become rate-limiting. In this review, we highlight recent findings regarding the role of nuclear mechanics in 3-D migration, including factors that govern nuclear deformability, and emerging mechanisms by which cells apply cytoskeletal forces to the nucleus to facilitate nuclear translocation. Intriguingly, the 'physical barrier' imposed by the nucleus also impacts cytoplasmic dynamics that affect cell migration and signaling, and changes in nuclear structure resulting from the mechanical forces acting on the nucleus during 3-D migration could further alter cellular function. These findings have broad relevance to the migration of both normal and cancerous cells inside living tissues, and motivate further research into the molecular details by which cells move their nuclei, as well as the consequences of the mechanical stress on the nucleus.},
author = {McGregor, Alexandra Lynn and Hsia, Chieh Ren and Lammerding, Jan},
doi = {10.1016/J.CEB.2016.01.011},
issn = {1879-0410},
journal = {Current opinion in cell biology},
keywords = {Alexandra Lynn McGregor,Animals,Cell Movement*,Cell Nucleus / physiology*,Chieh-Ren Hsia,Cytoskeleton,Humans,Jan Lammerding,Lamins / metabolism,MEDLINE,NCBI,NIH,NLM,National Center for Biotechnology Information,National Institutes of Health,National Library of Medicine,Neoplasm Metastasis,Neoplasms / pathology,PMC4887392,PubMed Abstract,Review,doi:10.1016/j.ceb.2016.01.011,pmid:26895141},
mendeley-groups = {Deformability},
month = {jun},
pages = {32--40},
pmid = {26895141},
publisher = {Curr Opin Cell Biol},
title = {{Squish and squeeze-the nucleus as a physical barrier during migration in confined environments}},
url = {https://pubmed.ncbi.nlm.nih.gov/26895141/},
volume = {40},
year = {2016}
}
@article{Vesperini2021,
abstract = {The immune system provides our defense against pathogens and aberrant cells, including tumorigenic and infected cells. Motility is one of the fundamental characteristics that enable immune cells to find invading pathogens, control tissue damage, and eliminate primary developing tumors, even in the absence of external treatments. These processes are termed “immune surveillance.” Migration disorders of immune cells are related to autoimmune diseases, chronic inflammation, and tumor evasion. It is therefore essential to characterize immune cell motility in different physiologically and pathologically relevant scenarios to understand the regulatory mechanisms of functionality of immune responses. This review is focused on immune cell migration, to define the underlying mechanisms and the corresponding investigative approaches. We highlight the challenges that immune cells encounter in vivo, and the microfabrication methods to mimic particular aspects of their microenvironment. We discuss the advantages and disadvantages of the proposed tools, and provide information on how to access them. Furthermore, we summarize the directional cues that regulate individual immune cell migration, and discuss the behavior of immune cells in a complex environment composed of multiple directional cues.},
author = {Vesperini, Doriane and Montalvo, Galia and Qu, Bin and Lautenschl{\"{a}}ger, Franziska},
doi = {10.1007/S12551-021-00787-9},
file = {::},
issn = {1867-2450},
journal = {Biophysical reviews},
keywords = {Doriane Vesperini,Franziska Lautenschl{\"{a}}ger,Galia Montalvo,MEDLINE,NCBI,NIH,NLM,National Center for Biotechnology Information,National Institutes of Health,National Library of Medicine,PMC8285443,PubMed Abstract,Review,doi:10.1007/s12551-021-00787-9,pmid:34290841},
mendeley-groups = {Deformability},
month = {apr},
number = {2},
pages = {185--202},
pmid = {34290841},
publisher = {Biophys Rev},
title = {{Characterization of immune cell migration using microfabrication}},
url = {https://pubmed.ncbi.nlm.nih.gov/34290841/},
volume = {13},
year = {2021}
}
@article{Tschumperlin2013,
abstract = {Fibroblast migration is essential to normal wound healing and pathological matrix deposition in fibrosis. This review summarizes our understanding of how fibroblasts navigate 2D and 3D extracellular matrices, how this behavior is influenced by the architecture and mechanical properties of the matrix, and how migration is integrated with the other principle functions of fibroblasts, including matrix deposition, contraction, and degradation. {\textcopyright} 2013 Int. Union Physiol. Sci./Am. Physiol. Soc.},
author = {Tschumperlin, Daniel J.},
doi = {10.1152/PHYSIOL.00024.2013},
file = {::},
issn = {15489213},
journal = {Physiology},
mendeley-groups = {Deformability},
month = {nov},
number = {6},
pages = {380},
pmid = {24186933},
publisher = {American Physiological Society},
title = {{Fibroblasts and the Ground They Walk On}},
url = {/pmc/articles/PMC3858213/ /pmc/articles/PMC3858213/?report=abstract https://www.ncbi.nlm.nih.gov/pmc/articles/PMC3858213/},
volume = {28},
year = {2013}
}
@article{Pogoda2022,
abstract = {In this work, we investigate whether stiffening in compression is a feature of single cells and whether the intracellular polymer networks that comprise the cytoskeleton (all of which stiffen with increasing shear strain) stiffen or soften when subjected to compressive strains. We find that individual cells, such as fibroblasts, stiffen at physiologically relevant compressive strains, but genetic ablation of vimentin diminishes this effect. Further, we show that unlike networks of purified F-actin or microtubules, which soften in compression, vimentin intermediate filament networks stiffen in both compression and extension, and we present a theoretical model to explain this response based on the flexibility of vimentin filaments and their surface charge, which resists volume changes of the network under compression. These results provide a new framework by which to understand the mechanical responses of cells and point to a central role of intermediate filaments in response to compression.},
author = {Pogoda, Katarzyna and Byfield, Fitzroy and Deptu{\l}a, Piotr and Cie{\'{s}}luk, Mateusz and Suprewicz, {\L}ukasz and Sk{\l}odowski, Karol and Shivers, Jordan L. and {Van Oosten}, Anne and Cruz, Katrina and Tarasovetc, Ekaterina and Grishchuk, Ekaterina L. and MacKintosh, Fred C. and Bucki, Robert and Patteson, Alison E. and Janmey, Paul A.},
doi = {10.1021/ACS.NANOLETT.2C00736/ASSET/IMAGES/LARGE/NL2C00736_0004.JPEG},
file = {:Users/ir.isturiz/Library/Application Support/Mendeley Desktop/Downloaded/Pogoda et al. - 2022 - Unique Role of Vimentin Networks in Compression Stiffening of Cells and Protection of Nuclei from Compressive Str.pdf:pdf},
issn = {15306992},
journal = {Nano Letters},
keywords = {AFM,compression-stiffening,compressive stress,intermediate filaments,vimentin},
mendeley-groups = {Deformability},
month = {jun},
number = {12},
pages = {4725--4732},
pmid = {35678828},
publisher = {American Chemical Society},
title = {{Unique Role of Vimentin Networks in Compression Stiffening of Cells and Protection of Nuclei from Compressive Stress}},
url = {https://pubs.acs.org/doi/full/10.1021/acs.nanolett.2c00736},
volume = {22},
year = {2022}
}
@article{Lorenz2022,
author = {Lorenz, C and K{\"{o}}ster, S},
doi = {10.1063/5.0099405},
file = {:Users/ir.isturiz/Library/Application Support/Mendeley Desktop/Downloaded/Lorenz, K{\"{o}}ster - 2022 - COLLECTIONS ARTICLES YOU MAY BE INTERESTED IN.pdf:pdf},
mendeley-groups = {Deformability},
title = {{COLLECTIONS ARTICLES YOU MAY BE INTERESTED IN}},
url = {https://doi.org/10.1063/5.0099405},
year = {2022}
}

@article{Lin2007,
abstract = {Microtubules are filamentous protein biopolymers found in eukaryotic cells. They form networks that guide active intracellular transport and support the overall cell structure. Microtubules are very rigid polymers, with persistence lengths as large as a millimeter. As such, they constitute an example of rodlike polymers, whose mechanical and rheological properties are as yet poorly understood. We measure the linear and nonlinear viscoelastic properties of isotropic solutions of purified microtubules, as well as networks permanently cross-linked with biotin-NeutrAvidin. In the linear regime both solutions and networks are soft elastic materials with elastic moduli on the order of a few pascals. The elastic moduli show a power-law dependence on tubulin concentration, c T , with G′ ∼ c T $\nu$ , where $\nu$ ≈ 1.4 for solutions and increases slightly to $\nu$ ≈ 1.6-1.8 for networks. At large deformations, we observe a concentration-dependent yield stress. The rheology of microtubule solutions cannot be explained by the Doi-Edwards model, which treats noninteracting rigid rods. Instead, they show behavior very similar to the permanently cross-linked networks, suggesting the presence of effective cross-linking even in pure microtubule solutions. We develop a simple model based on transient cross-linking interactions between microtubules to interpret the rheological response. We also calculate a lower bound estimate of the strength of this interaction. Our data provide a framework with which to understand the dynamics and mechanics of more physiological networks of microtubules with microtubule-associated cross-linking and motor proteins, and ultimately to understand the role of microtubules in cell mechanics.},
author = {Lin, Yi-Chia and Koenderink, Gijsje H and Mackintosh, Frederick C and Weitz, David A},
doi = {10.1021/ma070862l},
mendeley-groups = {Deformability},
title = {{Viscoelastic Properties of Microtubule Networks}},
year = {2007}
}

